Domain-decomposed Bayesian inversion based on local Karhunen-Lo\`{e}ve expansions

In many Bayesian inverse problems the goal is to recover a spatially varying random field. Such problems are often computationally challenging especially when the forward model is governed by complex partial differential equations (PDEs). The challenge is particularly severe when the spatial domain is large and the unknown random field needs to be represented by a high-dimensional parameter. In this paper, we present a domain-decomposed method to attack the dimensionality issue and the method decomposes the spatial domain and the parameter domain simultaneously. On each subdomain, a local Karhunen-Lo`eve (KL) expansion is constructed, and a local inversion problem is solved independently in a parallel manner, and more importantly, in a lower-dimensional space. After local posterior samples are generated through conducting Markov chain Monte Carlo (MCMC) simulations on subdomains, a novel projection procedure is developed to effectively reconstruct the global field. In addition, the domain decomposition interface conditions are dealt with an adaptive Gaussian process-based fitting strategy. Numerical examples are provided to demonstrate the performance of the proposed method.

==> Sections/2subdomains.tex <==
\subsection{Test problem 1: Two subdomains}
\label{sec:2_sub}
In this section, we consider the problem domain on the rectangular domain $\calD = [0,2]\times [0,1] \in \mathbb{R}^2$.
Let $\calD^{(1)} = [0,1] \times [0,1]$ and $\calD^{(2)} = [1,2]\times [0,1]$, and the interface is $\btau^{(1,2)} = \{ 1\} \times [0,1]$.
The comparison of the computational costs for solving the the global forward model and the local forward model are listed in Table \ref{table: forward_cost_2subdomains}. 
Take the correlation length to be $L=0.8$, the global KL takes 88 terms, and the local KL takes 48 terms. 
The groundtruth and the corresponding pressure field together with sensor placement are shown in Figure  \ref{fig:setup_2sub_0_8}.

Figure \ref{fig:inv_res_2_subdomains} shows the comparison the inversion results. The reference inversion result is shown in Fig. \ref{fig:inv_res_2_subdomains} (b), we can see that although several salient features of the groundtruth (a) are indeed captures by (b), the result is still unsatisfactory because it lacks details and needs to further refined.
Figure \ref{fig:inv_res_2_subdomains} (c) shows the assembled inversion result with \textit{exact} boundary condition specified and Figure \ref{fig:inv_res_2_subdomains} (d) shows the posterior mean estimate with GP-fitting boundary condition, we can see that even though the parallel MCMC gives result outperforms the global inversion, the uncertain boundary can still cause error.


\begin{figure}
\centering
\subfigure{
      \includegraphics[scale=0.3]{Figures/Test_8.000000e-01_L_7_mc_1_2_subdomains/Groundtruth_L_8.000000e-01.eps}
      %\label{fig:global_kle}
      }
\subfigure{
      \includegraphics[scale=0.3]{Figures/Test_8.000000e-01_L_7_mc_1_2_subdomains/pressure_field.eps}
      %\label{fig:stitched_kle}
      }
%\label{fig:random_field_reconstruction}
\caption{Setup of the inverse problem. Left: groundtruth permeability field used for generating the synthetic data. Right: pressure field corresponding to the groundtruth premeability field and the observations (black dots).}
\label{fig:setup_2sub_0_8}
\end{figure}

\begin{table}[!htp]
	\caption{Computational cost of the different scales forward model. (2 subdomains)} 
	\centering	
	\begin{tabular}{ccccc}  
		\hline
		Domain Area& Discretization   & DOF & Seconds &  Normalized Time\\ \hline
		Global & $65 \times 33$  & 2145 & 0.0125 &  $2.78$\\
		Local &$33 \times 33$ &1089&  0.0045& $1.00$ \\
		\hline
	\end{tabular}
	\label{table: forward_cost_2subdomains}
\end{table}


We run 100000 iterations in parallel MCMC, and we set the stepsize as $\beta = 0.07$ to encourage its convergence. 
The reference experiment we consider is the global forward model using the same cost of our proposed method. 
Therefore, we run 36000 MCMC iterations for the global case. 
And for all implementations of the MCMC algorithms, we set the burn-in rate as 0.1, that is, to keep only the last 10\% samples of total samples as the posterior samples. 

Figures \ref{fig:inv_res_2_subdomains} 

Figures 
\ref{fig:SSR_2subdomains} and \ref{fig:RMSE_2subdomains} show the convergence results of the local case and the global case respectively.
We can see that the local case outperform the global case in terms of convergence results.


%\begin{figure}
%\centering
%\subfigure[Groundtruth]{
  %    \includegraphics[scale=0.37]{Figures/Test_0_8_L_2_mc_1_2subdomains/Groundtruth_L_8.000000e-01.eps}
      %\label{fig:global_kle}
 %     }
%\subfigure[Assembled random field]{
 %     \includegraphics[scale=0.37]{Figures/Test_0_8_L_2_mc_0_2subdomains/Assemble_inverse_iter_200000.eps}
      %\label{fig:stitched_kle}
%      }
%\subfigure[Inversion using $\bF_C$]{
%    \includegraphics[scale = 0.37]{Figures/Test_0_8_L_2_mc_0_2subdomains/Global_mc_inverse_iter_200000.eps}
%    }
%\label{fig:random_field_reconstruction}
%\caption{Comparison of inversion results (Naive parallel MCMC algorithm).}
%\label{fig:setup_2sub_0_8}
%\end{figure}

%\begin{figure}
%\centering
%\subfigure[Groundtruth]{
 %     \includegraphics[scale=0.37]{Figures/Test_8.000000e-01_L_5_mc_1_2_subdomains/Groundtruth_L_8.000000e-01.eps}
      %\label{fig:global_kle}
 %     }
%\subfigure[Assembled random field]{
 %     \includegraphics[scale=0.37]{Figures/Test_8.000000e-01_L_5_mc_1_2_subdomains/Assemble_inverse_iter_100000.eps}
      %\label{fig:stitched_kle}
%      }
%\subfigure[Global inversion]{
%    \includegraphics[scale = 0.37]{Figures/Test_8.000000e-01_L_5_mc_1_2_subdomains/Global_fine_inverse_iter_36000.eps}
%    }
%\label{fig:random_field_reconstruction}
%\caption{Comparison of inversion results (Naive parallel MCMC algorithm).}
%\label{fig:setup_2sub_0_8}
%\end{figure}

\begin{figure}
\centering
\subfigure[Groundtruth]{
      \includegraphics[scale=0.3]{Figures/Test_8.000000e-01_L_6_mc_1_2_subdomains/Groundtruth_L_8.000000e-01.eps}
      %\label{fig:global_kle}
      }
\subfigure[Global inversion]{
    \includegraphics[scale = 0.3]{Figures/Test_8.000000e-01_L_6_mc_1_2_subdomains/Global_fine_inverse_iter_36000.eps}
    }
\subfigure[Assembled random field (with exact boundary condition)]{
      \includegraphics[scale=0.3]{Figures/Test_8.000000e-01_L_6_mc_1_2_subdomains/Assemble_inverse_iter_100000.eps}
      %\label{fig:stitched_kle}
      }
\subfigure[Assembled random field (with GP-fitting boundary)]{
    \includegraphics[scale = 0.3]{Figures/Test_8.000000e-01_L_7_mc_1_2_subdomains/Assemble_inverse_iter_100000.eps}
    }

%\label{fig:random_field_reconstruction}
\caption{Comparison of inversion results (Parallel MCMC algorithm).}
\label{fig:inv_res_2_subdomains}
\end{figure}

\begin{figure}
    \centering
    \subfigure[]{
    \includegraphics[scale = 0.25]{
    Figures/Test_8.000000e-01_L_7_mc_1_2_subdomains/SSR_obs_local_1.eps}
    }
    \subfigure[]{
    \includegraphics[scale = 0.25]{
    Figures/Test_8.000000e-01_L_7_mc_1_2_subdomains/SSR_obs_local_2.eps}
    }
    \subfigure[]{
    \includegraphics[scale = 0.25]{
    Figures/Test_8.000000e-01_L_7_mc_1_2_subdomains/SSR_obs_global.eps}
    }
    \caption{The convergence of the Markov chain. (a) the SSR of observable pressure values versus the MCMC iteration in the subdomain $\calD^{(1)}$; (b) the SSR of observable pressure values versus the MCMC iteration in the subdomain $\calD^{(2)}$; (c) the SSR of observable pressure values versus the MCMC iteration in the global domain $\calD$.}
    \label{fig:SSR_2subdomains}
\end{figure}

\begin{figure}
    \centering
    \subfigure[]{
    \includegraphics[scale = 0.25]{
    Figures/Test_8.000000e-01_L_7_mc_1_2_subdomains/RMSE_obs_local_1.eps}
    }
    \subfigure[]{
    \includegraphics[scale = 0.25]{
    Figures/Test_8.000000e-01_L_7_mc_1_2_subdomains/RMSE_obs_local_2.eps}
    }
    \subfigure[]{
    \includegraphics[scale = 0.25]{
    Figures/Test_8.000000e-01_L_7_mc_1_2_subdomains/RMSE_obs_global.eps}
    }
    \caption{The convergence of the Markov chains with the same cost. (a) the RMSE of observable pressure values versus the MCMC iteration in the subdomain $\calD^{(1)}$; (b) the RMSE of observable pressure values versus the MCMC iteration in the subdomain $\calD^{(2)}$; (c) the RMSE of observable pressure values versus the MCMC iteration in the global domain $\calD$.}
    \label{fig:RMSE_2subdomains}
\end{figure}

\begin{figure}
    \centering
    \subfigure[Posterior mean at iteration 10000]{
    \includegraphics[scale = 0.3]{
    Figures/Test_8.000000e-01_L_7_mc_1_2_subdomains/Assemble_inverse_iter_10000.eps}
    }
    \subfigure[Posterior mean at iteration 50000]{
    \includegraphics[scale = 0.3]{
    Figures/Test_8.000000e-01_L_7_mc_1_2_subdomains/Assemble_inverse_iter_50000.eps}
    }
    \subfigure[Posterior mean at iteration 100000]{
    \includegraphics[scale = 0.3]{
    Figures/Test_8.000000e-01_L_7_mc_1_2_subdomains/Assemble_inverse_iter_100000.eps}
    }
    \caption{The states evoluation during iterations in the Markov chain.}
    % \label{fig:my_label}
\end{figure}

\begin{figure}
    \centering
    \subfigure[Posterior estimate mean]{
    \includegraphics[scale = 0.37]{
    Figures/Test_8.000000e-01_L_7_mc_1_2_subdomains/Global_fine_inverse_iter_36000.eps}
    }
    %\subfigure[Posterior estimate variance]{
    %\includegraphics[scale = 0.37]{
    %Figures/Test_8.000000e-01_L_7_mc_1_2_subdomains/Variance_Global_fine_inverse_iter_36000.eps}
    %}
    \caption{Caption}
    % \label{fig:my_label}
\end{figure}

==> Sections/3subdomains_high.tex <==
\subsection{Test problem 2: high-dimensional case on three subdomains}
\label{sec:3_sub_high}


==> Sections/analysis.tex <==
\subsection{Analysis}
Denote the posterior mean of local random variables as $\mathbb{E}[\bxi_l^{(i)}]$ and
suppose the inversion accuracy is bounded as 
\[
\|\mathbb{E}[\bxi_l^{(i)}] - \bxi_l^{(i)} \|_2 \le \delta_{l}^{(i)}\,,\quad i=1,\ldots,M, l=1,\ldots,d^{(i)}\,,
\]
where $\|\cdot\|_2$ denotes the convential vector 2-norm, 
then the accuracy of assembled global random variables is bounded by
\begin{align*}
    \|\mathbb{E}[\widehat{\bxi}_j] - \widehat{\bxi}_j\|_2 
    & = \left\| \frac{1}{\sqrt{\lambda_j}}\sum_{i=1}^M\sum_{l=1}^{d^{(i)}}\sqrt{\lambda_l^{(i)}}[\mathbb{E}[\bxi_l^{(i)}] - \bxi_l^{(i)}]\int_{\calD^{(i)}} \psi_l^{(i)}(\bx)\psi_j(\bx)\dif \bx\right\|_2 \\
    & \le \frac{1}{\sqrt{\lambda_j}}\sum_{i=1}^M\sum_{l=1}^{d^{(i)}}\sqrt{\lambda_l^{(i)}}\|\mathbb{E}[\bxi_l^{(i)}] - \bxi_l^{(i)} \|_2\int_{\calD^{(i)}} \psi_l^{(i)}(\bx)\psi_j(\bx)\dif \bx \\
    & \le \frac{1}{\sqrt{\lambda_j}}\sum_{i=1}^M \sum_{l=1}^{d^{(i)}}\sqrt{\lambda_l^{(i)}} \delta_l^{(i)}\,,\quad j=1,\ldots,d\,.
\end{align*}
We define the posterior mean assembled random filed via the posterior mean random variables, i.e.,
\begin{align*}
  \mathbb{E}[\widehat{\ba}(\bx,\widehat{\bxi})]:= \ba_0(\bx) + \sum_{j=1}^d \sqrt{\lambda_j}\psi_j(\bx) \mathbb{E}[\widehat{\bxi}_j]\,,
\end{align*}
then the accuracy of the posterior assembled random filed is given by 
\begin{align*}
    & \| \mathbb{E}[\widehat{\ba}(\bx,\widehat{\bxi}(\bomega))] - \ba(\bx,\bxi(\bomega))\|_\calD^2\\
    & \quad =  \| \mathbb{E}[\widehat{\ba}(\bx,\widehat{\bxi}(\bomega))] - \widehat{\ba}(\bx,\widehat{\bxi}(\bomega)) + 
    \widehat{\ba}(\bx,\widehat{\bxi}(\bomega))
    - \ba(\bx,\bxi(\bomega))\|_\calD^2\\
    & \quad     \le \| \mathbb{E}[\widehat{\ba}(\bx,\widehat{\bxi}(\bomega))] - \widehat{\ba}(\bx,\widehat{\bxi}(\bomega))\|_\calD^2 + 
    \|
    \widehat{\ba}(\bx,\widehat{\bxi}(\bomega))
    - \ba(\bx,\bxi(\bomega))\|_\calD^2\\
    %& \le d \left(\sum_{i=1}^M \sum_{l=1}^{d^{(i)}}\sqrt{\lambda_l^{(i)}}\delta_l^{(i)} \right)^2 + d \left(\sum_{i=1}^M \sum_{l=d^{(i)}}^{+\infty}\sqrt{\lambda_l^{(i)}}\bxi_l^{(i)}(\bomega) \right)^2 \\
    & \le d\sum_{i=1}^M \left(
    \sum_{l=1}^{d^{(i)}}\lambda_l^{(i)}(\delta_l^{(i)})^2 + \sum_{l=d^{(i)}+1}^{\infty}\lambda_l^{(i)}
    (\bxi_l^{(i)}(\bomega))^2
    \right)
\end{align*}
where the first term 
\begin{align*}
   & \| \mathbb{E}[\widehat{\ba}(\bx,\widehat{\bxi}(\bomega))] - \widehat{\ba}(\bx,\widehat{\bxi}(\bomega))\|_\calD^2 
   = 
   \left\| \sum_{j=1}^d \sqrt{\lambda_j}\psi_j(\bx) (\mathbb{E}[\widehat{\bxi}_j(\bomega)] - \widehat{\bxi}_j(\bomega)) \right\|_\calD^2\\
   &\quad  \le \sum_{j=1}^d \left\|  \sqrt{\lambda_j}\psi_j(\bx) (\mathbb{E}[\widehat{\bxi}_j(\bomega)] - \widehat{\bxi}_j(\bomega)) \right\|_\calD^2\\
   & \quad =\sum_{j=1}^d \int_{\calD} \left(\sqrt{\lambda_j}\psi_j(\bx) (\mathbb{E}[\widehat{\bxi}_j(\bomega)] - \widehat{\bxi}_j(\bomega))\right)^2 \dif \bx \\
   & \quad =\sum_{j=1}^d \lambda_j \left(\frac{1}{\sqrt{\lambda_j}}\sum_{i=1}^M \sum_{l=1}^{d^{(i)}}\sqrt{\lambda_l^{(i)}}\delta_l^{(i)} \right)^2 \int_{\calD}\psi_j(\bx)^2\dif \bx \\
   & \quad = \sum_{j=1}^d \left(\sum_{i=1}^M \sum_{l=1}^{d^{(i)}}\sqrt{\lambda_l^{(i)}}\delta_l^{(i)} \right)^2
    = d \left(\sum_{i=1}^M \sum_{l=1}^{d^{(i)}}\sqrt{\lambda_l^{(i)}}\delta_l^{(i)} \right)^2\\
    & \quad \le d \sum_{i=1}^M \sum_{l=1}^{d^{(i)}}\lambda_l^{(i)}(\delta_l^{(i)})^2\,,
\end{align*}
and the second term is given in \eqref{eq:field_error}.


For the purpose of comparison, we use the inversion result given by the global model as reference. 

==> Sections/method.tex <==
\section{Problem setup}
\label{sec:problem_setup}
%In this section, we provide an overview of the Bayesian framework and the KLE parameterization.
In this section, we review the general description of  Bayesian formulation for inference and detailed settings for KL expansion parameterization for PDEs with random inputs.

\subsection{Bayesian inverse problem}
%Given a physical system, 
Letting $\btheta$ denote a $N$-dimensional parameter of interest and $\bd\in \mathbb{R}^{n} (n\ll N)$ denote  $n$-dimensional observational data, we want to estimate  $\btheta$ from $\bd$.  %the unknown $\btheta$ of a physical system can be a spatially distributed parameters.
We assume that there exists a forward model $\bF$ that maps the unknown parameter $\btheta$ to the data $ \bd$:
\begin{equation}
    \bd = \bF(\btheta)+ \bepsilon\,,
\end{equation}
where $\bepsilon$ denotes the random observation error and 
its probability density function is denoted by $\pi_{\bepsilon}(\bepsilon)$. 
%In the Bayesian setting, both the unknown input $\btheta$ and the observation are considered as random variables. 
Then, the likelihood function which characterizes the relationship between observations and forward models can be defined as 
\[
\bL(\bd|\btheta) = \pi_{\bepsilon}(\bd - \bF(\btheta))\,.
\]
When the measurement noise is assumed to be mean-zero white additive Gaussian noise with covairance matrix $\bSigma$, i.e.,
$\bepsilon\sim \mathcal{N}(\bm{0},\bSigma)$, 
the likelihood function is then proportional to the \textit{the data-misfit functional} $\eta(\btheta;\bd)$, %that is,
i.e.,
\begin{equation*}
	\label{eq:likelihood}
	\bL(\bd|\btheta) \propto \exp(-\eta(\btheta;\bd))
\end{equation*}
with $\eta(\btheta;\bd) := \frac{1}{2}(\bd - \bF(\btheta))^T \bSigma^{-1}(\bd - \bF(\btheta))$.
Given a prior distribution $\pi_0(\btheta)$ of $\btheta$, based on the Bayes' rule,  %combining the observed data yields 
the posterior distribution of $\btheta$ can be written as
\begin{equation}
	\label{eq:bayes}
	\pi(\btheta|\bd) = \frac{ \overbrace{\bm{L}(\bd|\btheta)}^{\text{likelihood}}
		\overbrace{\pi_0(\btheta)}^{\text{prior}}
	}
	{
		\underbrace{
			\pi(\bd)}_{\text{evidence}}}
	\propto \bL(\bd|\btheta) \pi_0(\btheta)
	\,,
\end{equation}
where the evidence $\pi(\bd)$ in \eqref{eq:bayes} is usually viewed as a normalization constant for a well-defined probability distribution. 
% The posterior distribution $\pi(\btheta|\bd)$ is often referred to as the solution of the Bayesian inverse problems. 
The posterior distribution is usually analytically intractable, and therefore sampling methods including Markov chain Monte Carlo methods (MCMC) \cite{kass1998markov, gamerman2006markov, robert2013monte, haario2001adaptive, haario2006dram} and Variational Inference (VI) \cite{blei2017variational}  are intensively used.
A Markov chain is a sequence of samples where the next state only depends on the previous state, which is known as the Markov property, and the move from the current state towards the next state is defined through some transition operator.
The MCMC method constructs a Markov chain whose equilibrium distribution (also known as the stationary distribution) of the chain, is set to be the target distribution.
In the context of Bayesian inversion, we set the traget distribution to be the posterior distribution. 
To ensure the convergence towards the target distribution, the detailed balance condition has to be satisfied.
The standard Metropolis-Hastings \cite{metropolis1953equation, hastings1970monte} 
algorithm works as follows.
Starting from a randomly chosen initial state, for current state $\btheta^{j}$, a candidate state $\btheta^{\star}$ is drawn from some proposal distribution $Q(\cdot|\btheta^{j})$, 
and then the candidate state is accepted with the probability of an
acceptance rate denoted by $\alpha(\btheta^{\star},\btheta^j)$. 
%the Metropolis Hastings step accepts the proposal with the probability of a %computed
%acceptance rate. %$\alpha(\btheta^{\star},\btheta^j)$.
The proposal distribution and the acceptance probability define the transition operator, i.e., $h(\btheta^{\star},\btheta^j) = Q(\btheta^{\star}|\btheta^j) \alpha(\btheta^{\star},\btheta^j).$
The detailed balance condition is given through the transition operator,  
\[
\pi(\btheta|\bd) h(\btheta^j,\btheta^{\star}) = \pi(\btheta^{\star}|\bd) h(\btheta^{\star},\btheta^j)\,.
\]
To guarantee that the detailed balance condition is satisfied, the acceptance probability can be defined as 
\[
\alpha(\btheta^{\star},\btheta^j) = \min\left\{1,
\frac{Q(\btheta^{j}|\btheta^{\star})\bL(\bd|\btheta^{\star})\pi_0(\btheta^{\star})}{Q(\btheta^{\star}|\btheta^{j})\bL(\bd|\btheta^{j})\pi_0(\btheta^{j})}\right\}\,.
\]
However, Markov chains can be trapped by local modes and long mixing times are typically required.
The standard MH (Metropolis-Hastings) algorithm is summarized in Algorithm \ref{alg:MHMCMC}.


\begin{algorithm}[!ht]
    \caption{The standard MH algorithm}
    \label{alg:MHMCMC}
    \begin{algorithmic}[1]
        \REQUIRE{Likelihood function $\bL(\bd|\cdot)$, proposal distribution $Q(\cdot|\cdot)$, prior distribution $\pi_0(\cdot)$, maximum iteration number MAX-ITER, observation data $\bd$, burn-in length $n_{\text{burn-in}}$}
        \STATE{\textbf{Initialization:} Randomly choose the initial state $\btheta^{1}$.}
    \FOR{$j=1,\ldots,\text{MAX-ITER}-1$}
    \STATE{Draw a proposal state $\btheta^{\star}$ from the proposal distribution $Q(\cdot|\btheta^{j})$.}
    \STATE{Compute the acceptance ratio $
\alpha = \min\left\{1,
\frac{Q(\btheta^{j}|\btheta^{\star})\bL(\bd|\btheta^{\star})\pi_0(\btheta^{\star})}{Q(\btheta^{\star}|\btheta^{j})\bL(\bd|\btheta^{j})\pi_0(\btheta^{j})}\right\}$.}
    \STATE{Draw $\rho$ from a uniform distribution $u \sim \mathcal{U}[0,1]$.}
    \IF{$\rho<\alpha$}
    \STATE{
    Accept the proposal state $\btheta^{j+1} = \btheta^\star$.
    }
    \ELSE
    \STATE{Reject the proposal and let $\btheta^{j+1} = \btheta^{j}$.}
    \ENDIF
    \ENDFOR
    \ENSURE{ Posterior samples $\{\btheta^j\}_{j=n_{\text{burn-in}}}^{\text{MAX-ITER}}$}
    \end{algorithmic}
\end{algorithm}

\subsection{PDEs with random inputs and parameterization}
This section presents the detailed setting of the forward model considered in the paper.
First, let $\mathcal{P}=(\Omega, \Sigma_{\Omega}, \mu_{\Omega})$ be a probability space, where $\Omega$ is the set of events, $\Sigma_{\Omega}$ is a sigma-algebra over $\Omega$ and $\mu_{\Omega}$ is a probability measure.
We denote the expectation operator as 
\[
\mathbb{E}[\bkappa] = \int_{\Omega}\bkappa(\bomega) \dif \mu_{\Omega}(\bomega)\,,
\]
for arbitrary function $\bkappa(\cdot)$ and event $\bomega\in\Omega$, 
and $L_2(\Omega)$ the space of second-order random variables, i.e., $L_2(\Omega):= \{\bkappa|\mathbb{E}[\bkappa^2]<+\infty \}$.
Moreover, 
let $\calD$  denote a physical domain (a subset of $\mathbb{R}^2$ or $\mathbb{R}^3$) which is  bounded, connected and with a
polygonal boundary $\partial \calD$,
and $\bx\in \calD$ denote a spatial variable. 
%Moreover, 
%consider a bounded spatial domain $\calD$ (a subset of $\mathbb{R}^2$ or $\mathbb{R}^3$). 
%\subset \mathbb{R}^{\mathbf{d}} (\mathbf{d}= 1,2,3)$ with polygonal boundary $\partial \calD$.
We denote $L_2(\calD)$ the space of square integrable functions $L_2(\calD) :=\{ f| \int_{\calD}f^2 < +\infty \}$, and $\|\cdot\|_{\calD}$ the norm in $L_2(\calD)$ which is induced by inner product 
\[
\forall f\in L_2(\calD)\,,\quad
\|f\|_{\calD}^2 = \langle f,f\rangle_{\calD} =\int_{\calD} f(\bx)^2\dif \bx\,.
\]
Finally, we denote by $L_2(\calD,\Omega)$ the space of real-valued second-order processes $\bkappa: \calD \times \Omega \to \mathbb{R}$ such that $\bkappa(\bx,\cdot)\in L_2(\calD)$ and  $\bkappa(\cdot, \bomega) \in L_2(\Omega)$.
The physics of problems considered 
are governed by 
a PDE over the spatial domain $\calD$ and
boundary conditions on the boundary $\partial \calD$,
which are stated as: 
find
$\bu(\bx,\bomega)$ mapping $\calD\times \Omega$ to $\mathbb{R}$, such that
%In this paper, we consider the following PDE system defined in $\calD$ with random input, 
\begin{equation*}
	\label{eq:original_pde}
\begin{aligned}
	&\mathcal{L}(\bx,\bu; \bkappa(\bx,\bomega)) = f(\bx,\bkappa(\bx,\bomega))\,,\quad \bx \in \calD\,,\\	&\mathcal{B}(\bx,\bu; \bkappa(\bx,\bomega)) = g(\bx,\bkappa(\bx,\bomega))\,,\quad \bx \in \partial \calD\,, 
\end{aligned}
\end{equation*}
where $\mathcal{L}$ is a differential operator and $\mathcal{B}$ is a boundary condition operator, both of which are dependent on a random process  $\bkappa(\bx,\bomega)$. 
%and $\bkappa(\bx,\bomega)$ denotes the unknown spatial-varying random process.
Here $f$ is the source term 
%which is usually assumed to be deterministic 
and $g$ specifies the boundary condition.
%In addition, $\bkappa(\bx,\bomega)$ denotes the unknown spatial-varying random process on the physical domain where $\bx$ denotes spatial location in the domain $\mathcal{D}$ and $\bomega$ defines the randomness of the random process. 
%Given a realization of $\bkappa$,  approximations of $\bu$ can be obtained by solving the deterministic version of \eqref{eq:original_pde} with standard numerical methods (e.g., finite element methods \cite{elman14finite}) on a set of discretized grid points.

Generally, the random field $\bkappa(\bx,\bomega)$ is infinite-dimensional and needs to be parameterized.
As the truncated Karhunen-Lo\`{e}ve (KL) expansion \cite{ghanem2003stochastic, spanos1989stochastic}  is an optimal representation of random processes in the mean squared error sense, we focus on this expansion.
Letting $\ba_0(\bx)$ be the mean function of $\bkappa(\bx,\bomega)$, the covariance function $C(\bx,\by):\calD\times \calD\to \mathbb{R}$ is defined as 
\[
	C(\bx,\by) = \mathbb{E}[(\bkappa(\bx,\bomega) - \ba_0(\bx))(\bkappa(\by,\bomega) - \ba_0(\by))]\,,\quad \bx,\by \in \mathcal{D}\,.
\]
We can express the covariance function as $C(\bx, \by) = \sigma(\bx) \sigma(\by) \rho(\bx,\by)$, where $\sigma: \calD \to \mathbb{R}$ is the standard deviation function of the random field and $\rho: \calD\times \calD \to [-1,1]$ is its autocorrelation coefficient function.
Let $\{\lambda_i,\psi_i(\bx)\}_{i=1}^{\infty}$ be the eigenvalues and the associated orthonormal eigenfunctions of the covariance function, that is, they satisfy 
\begin{equation*}
    \int_{\calD} C(\bx,\by) \psi_i(\bx)\dif \bx = \lambda_i\psi(\by)\,,
\end{equation*}
and
\begin{equation*}
    \int_{\calD} \psi_i(\bx)\psi_j(\bx)\dif \bx = \delta_{ij}\,,
\end{equation*}
where $\delta_{ij}$ denotes the Kronecker delta, and here we assume that the eigenvalues are ordered in decreasing magnitude.
By Mercer's Theorem, the covariance function has the following spectral decomposition, 
\[
C(\bx,\by)  =\sum_{i=1}^{\infty} \lambda_i \psi_i(\bx) \psi_i(\by)\,.
\]
According to the decomposition, it can be seen that 
$
 \sum_{i=1}^{\infty} \lambda_i = \int_{\calD} C(\bx,\bx)\dif \bx\,.
$
Based on the eigen-decomposition of the covariance function, the KL expansion provides a representation in terms of infinite number of random variables,
\begin{equation}
\label{eq:kle_inf}
	\bkappa(\bx,\bomega) = 
	\ba^{\infty}(\bx,\bxi(\bomega)):=
	\ba_0(\bx) + \sum_{i=1}^{\infty}\sqrt{\lambda_i} \psi_i(\bx) \bxi_i(\bomega)\,,\quad \bx\in \mathcal{D}\,,
\end{equation}
where $\{\bxi_i(\bomega)\}_{i=1}^{\infty}$ are the uncorrelated random variables which controls the randomness of the random filed.
In this paper, we refer $\ba(\bx,\bxi(\bomega)) - \ba_0(\bx)$ to as the \textit{centralized} random field of $\ba(\bx,\bxi(\bomega))$.
Moreover, note that the centralized field $\ba^{\infty}(\bx,\bxi(\bomega))-\ba_0(\bx)$ lies in the Hilbert space spanned by orthonormal bases $\{\psi_i(\bx)\}_{i=1}^{\infty}$ 
%.
%The associated normalized eigenfunctions $\{\psi_i(\bx)\}_{i=1}^{\infty}$ 
(which form a complete orthonormal basis of $L_2(\calD)$).
For a given fixed random field  $\bkappa(\bx,\bomega)$, 
the corresponding random variables can be given via the orthonormality of eigenfunctions, 
\begin{equation}
	\label{eq:kle_xi}
	\bxi_j(\bomega) = \frac{1}{\sqrt{\lambda_j}} \int_{\calD} [\bkappa(\bx,\bomega)) - \ba_0(\bx)] \psi_j(\bx) \dif \bx\,,\quad j =1,\ldots\,,
\end{equation}
and satisfy $\mathbb{E}[\bxi_i] =0 $ and $\mathbb{E}[\bxi_i \bxi_j] =\delta_{ij}.$
For practical implementations, \eqref{eq:kle_inf} can be truncated with a finite number of terms, 
\[
\ba^{\infty}(\bx,\bxi(\bomega)) \approx \ba^{\text{KL}}(\bx, \bxi(\bomega)) = \ba_0(\bx) + \sum_{i=1}^{d}\sqrt{\lambda_i} \psi_i(\bx) \bxi_i(\bomega) \,,\quad \bx\in \mathcal{D}\,.
\]
The truncation level $d$ depends on the decay rate of eigenvalues which is related to the correlation length of the random field $\ba$.
Usually, we select $d$ such that at least $\delta_{\text{KL}}$ of the total variance is captured for the pre-set threshold $\delta_{\text{KL}}$, i.e., $(\sum_{i=1}^d \lambda_i)/(|\calD|\sigma^2)>\delta_{\text{KL}}$, where $|\calD|$ denotes the area of the domain $\calD$.
For a continuous covariance  function, the truncated KL expansion converges in the mean square sense uniformly \cite{le2010spectral} on $\calD$, i.e., 
\[
\lim_{d\to \infty} \sup_{\bx\in \calD} 
\mathbb{E}\left(
\ba^{\infty}(\bx,\bxi(\bomega)) - \ba_0(\bx) - \sum_{i=1}^d \sqrt{\lambda_i}\psi_i(\bx)\bxi_i(\bomega)
\right)^2  =0\,.
\]
When the random field has short correlation length, the parameterized inputs $\ba^{\text{KL}}(\bx,\bxi(\bomega))$ will have a large number of terms \cite{chen2015local, hou2017exploring}, and consequently, such inverse problem is in general highly ill-posed. It makes the inverse problem very time-consuming and computationally expensive to solve, as most of the existing numerical methods suffers from the curse of dimensionality.
In the sequel, we will drop the superscript $\cdot^{\text{KL}}$ and refer the truncated $\ba(\bx,\bxi(\bomega))$ as the KL expansion in the absence of ambiguity. 

After parameterization over the random field, the original governing equation is then transformed into a parameterized PDE system,
\begin{equation}
	\label{eq:parameterized_pde}
\begin{aligned}
	&\mathcal{L}(\bx,\bu; \ba(\bx,\bxi(\bomega))) = f(\bx,\ba(\bx,\bxi(\bomega)))\,,\quad \bx \in \calD\,,\\	&\mathcal{B}(\bx,\bu; \ba(\bx,\bxi(\bomega))) = g(\bx,\ba(\bx,\bxi(\bomega)))\,,\quad \bx \in \partial \calD\,, 
\end{aligned}
\end{equation}

Often, solution $\bu$ and the random field $\ba$ are discretized by a random vector $\mathbf{x}:=[\mathbf{x}_1,\mathbf{x}_2,\ldots,\mathbf{x}_N]\in \mathbb{R}^N$ using numerical methods such as finite element methods \cite{elman14finite}.
Here $\mathbf{x}_i$ denotes the $i$-th location of given physical grid points and $N$ is the number of grid points (or known as the finite element degrees of freedom (DOF)).

In this work, assume that some noisy and indirect data $\bd\in\mathbb{R}^n$ is given by 
\begin{equation}
	\label{eq:obs}
\bd = \mathcal{O}(\bu) + \bepsilon\,,
\end{equation}
where $\mathcal{O}$ is the observation operator which extracts partial noisy observations 
mapping from the solution $\bu$ to the locations of sensors, 
we are interested in recovering the high-dimensional unknown parameter that represents the discretized random filed, i.e., $\btheta = \ba(\bx,\bxi(\bomega))$.  

The PDE system \eqref{eq:parameterized_pde} together with the observation model \eqref{eq:obs} defines a \textit{global forward model} which maps the unknown input into the observations, 
\begin{equation}
	\label{eq:forward}
	\bd = \bF(\ba(\bx,\bxi(\bomega))) + \bepsilon\,.
\end{equation}

\section{Domain-decomposed Parameterization}
In this section, we discuss KL expansion parameterization for the spatial-varying random field in the global domain and the local domain respectively.
Global KL expansion
characterizes an infinite-dimensional function with a set of finite independent random variables.
However, there are still many terms when the correlation length is short. Therefore, we turn to domain decomposition for a further possible dimension reduction.

The attempt to enable parallelization and enlarge representation capacity through domain decomposition methods is not new.
Japtap et al. \cite{jagtap2020conservative} proposed conservative physical-informed neural networks (cPINNs), which employ domain decomposition technique in the computation domain.
By considering smaller sub-domain, 
the computational efficiency is improved due to the parallelized property.
Also, the neural network within each subdomain allows simpler and more shallow structure.
Moreover, a generalized framework named eXtended PINNs (XPINNs), which is also based on domain decomposition, is proposed \cite{jagtap2020extended}.
In \cite{shukla2021parallel}, authors develop a distributed PINN framework based on cPINNs and XPINNs to achieve better performance in multi-scale and multi-physics problems. 

Typically, the computation of eigenvalues requires the solution of integral problems,
and analytical solutions are only available for a specific form of covariance functions, see \cite{spanos1989stochastic} for more details.
In this paper, the numerical examples we consider only are restricted in the case where analytical solutions of the integral problem are available, and we remark here that other covariance functions with more complicated domains can be readily used. 

\subsection{Local KL expansion parameterization}
Divide the physical domain $\calD$ into a set of subdomains $\calD^{(i)}, i=1,\ldots,M$, i.e., $\calD = \cup_{i=1}^M \calD^{(i)}$.
\footnote{In this paper, the superscript $ \cdot^{(i)}$ represents variables or functions related to the subdomain $\calD^{(i)}$, the superscript $ \cdot^{i}$ represents sample $i$, and the subsript $\cdot_{i}$ denotes the component $i$ of a vector.} 
We consider the case where the intersection of two subdomains can only be a connected interface with positive $(\mathbf{d}-1)$-dimensional measure or an empty set.
For a fixed random input $\bkappa(\bx,\bomega)$, 
differential operator together with a given boundary condition defines a complete deterministic system. 
For a subdomain $\calD^{(i)}$, let $\partial \calD^{(i)}$ denote all of its boundaries, 
among these boundaries, some boundaries is well defined via global boundary condition while some are adjoined with boundaries of other subdomains. 
We use $\btau^{(ij)}$ to represent the interface of $\calD^{(i)}$ and $\calD^{(j)}$.

More specifically, for $i=1,\ldots,M$, consider
\begin{align}
	&\mathcal{L}^{(i)} (\bx,u^{(i)};\bkappa(\bx,\bomega)) = f(\bx,\bkappa)\,,\quad \bx\in \calD^{(i)}\,,\label{eq:sub_problem} \\
	&\mathcal{B}^{(i)}(\bx, u^{(i)};\bkappa(\bx,\bomega)) = g^{(i)}(\bx,\bkappa)\,,\quad \bx\in \partial \calD^{(i)}\cap \partial \calD\,, \label{eq:sub_problem_boundary}\\
	& \mathcal{B}^{(i,j)} (\bx, u^{(i)}; \bkappa(\bx,\bomega)) = g^{(ij)}(\bx,\bkappa)\,,\quad \bx \in \btau^{(i,j)}\,,\quad j\ne i\label{eq:sub_problem_interface}\,.
\end{align}
Here $u^{(i)}$ denotes the restriction of $u$ to $\calD^{(i)}$.
We assume that each subdomain problem can be well defined and solved independently with the specified boundary condition.
Also, we assume that the collection of the subdomain solutions is equivalent to that of the original problem in the global domain, i.e.,
\begin{equation*}
	u(\bx,\bomega) = \sum_{i=1}^M u^{(i)}(\bx,\bomega) \mathbb{I}_{\calD^{(i)}}(\bx)\,,
\end{equation*}
where $\mathbb{I}_{A}(x)$ is the indicator function satisfying
\[
\mathbb{I}_A(x) = \begin{cases}
	1\,,\quad \text{if }x\in A\,,\\
	0 \,, \quad \text{otherwise}\,.
\end{cases}
\]
In \eqref{eq:sub_problem_interface}, $\mathcal{B}^{(ij)}$ and $g^{(i,j)}$ together describes the coupling relation between two neighbouring sub-domains $\calD^{(i)}$ and $\calD^{(j)}$. 
Naturally, the concrete forms of $\mathcal{B}^{(i,j)}$ and $g^{(i,j)}$ rest with the original problem. For example, for subdomain $\calD^{(i)}$, we can specify Dirichlet boundary conditions on the interface $\btau^{(i,j)}$ for $j\ne i$, i.e., 
\[
u^{(i)} = g^{(i,j)}(\bx,\bkappa)\,,\quad \bx \in \btau^{(i,j)}\,, j\ne i\,.
\]
In this case, $g^{(i,j)}$ is defined as the Dirichelt condition for this sub-problem.



In each subdomain $\calD^{(i)}$, $i=1,\ldots,M$, the local random field can be defined via the restriction of the subdomain over the global domain, for $\bx\in \calD^{(i)}$,
\begin{equation}
	\label{eq:local_kle}
	\bkappa^{(i)}(\bx,\bomega) = \bkappa(\bx,\bomega) \mathbb{I}_{\calD^{(i)}}(\bx)
	= \left(\ba_0(\bx) + \sum_{j=1}^{\infty} \sqrt{\lambda_j}\psi_j(\bx) \bxi_j(\bomega) \right)\mathbb{I}_{\calD^{(i)}}(\bx) \,.
\end{equation}
Naturally, the mean function of the local random field follows the same distribution. 
Also, we can see that the local field follows the same distribution as the original random field with the same covariance function $C(\bx,\by)$. 
Therefore, local eigenpairs $\{\lambda_j^{(i)}, \psi_j^{(i)}\}$ over the local domain $\calD^{(i)}$ satisfy the integral equation.  
We can then define the KL expansion locally.

\begin{definition}[Local KL expansion of $\bkappa(\bx,\bomega)$]
Suppose $\bkappa(\bx,\bomega)$ is the global random field and $\ba(\bx,\bxi(\bomega))$ is the truncated KL expansion over the global domain $\calD$ with the covariance function $C(\bx,\by)$ and the mean function $\ba_0(\bx)$.
Then the local KL expansion over the subdomain $\calD^{(i)}$ for the local random filed $\bkappa^{(i)}(\bx,\bomega)$ is given by  
\[
\bkappa^{(i)}(\bx,\bomega) =
\ba^{(i),\infty}(\bx,\bxi^{(i)}(\bomega)) = \ba_0^{(i)}(\bx) + \sum_{l=1}^{\infty}\sqrt{\lambda_l^{(i)}}\psi_l^{(i)}(\bx)\bxi_l^{(i)}(\bomega)\,,
\quad \bx\in \calD^{(i)}\,,
\]
where the mean function of the local random field satisfies 
 $\ba_0^{(i)}(\bx) = \ba(\bx)\mathbb{I}_{\calD^{(i)}}(\bx)$.
The local eigenpairs $\{\lambda_l^{(i)}, \psi_l^{(i)}\}$ over the local domain $\calD^{(i)}$ can be defined
\begin{equation}
\label{eq:local_eigenpair}
	\int_{\calD^{(i)}} C(\bx,\by) \psi_l^{(i)}(\bx) \dif \bx = \lambda_l^{(i)} \psi_l^{(i)}(\by)\,,
	\quad \|\psi_l^{(i)}\|_{\calD^{(i)}}^2=1\,,
	l =1,2,\ldots,\quad \bx,\by\in \calD^{(i)}\,,
\end{equation}
where $\|\cdot\|_{\calD^{(i)}}^2$ denotes the natural restriction of the norm in $L_2(\calD)$ to the subdomain $\calD^{(i)}$.
The local random variables $\bxi^{(i)}(\bomega) = [\bxi^{(i)}_l(\bomega)]_{l=1,\ldots,
\infty}$ for the local KL expansion $\ba^{(i)}(\bx,\bxi^{(i)}(\bomega))$ can be defined by its eigenvalues and eigenfunctions,
\begin{equation}
\label{eq:local_para}
	\bxi_l^{(i)}(\bomega) = \frac{1}{\sqrt{\lambda_j^{(i)}}} \int_{\calD^{(i)}} [\ba^{(i),\infty}(\bx,\bxi^{(i)}(\bomega)) - \ba_0^{(i)}(\bx)] \psi_l^{(i)}(\bx) \dif \bx\,,\quad l=1,\ldots\,.
\end{equation}
Similarly, we can truncate the local domain with finite terms.
To sum up, the truncated local KL expansion for $\bkappa^{(i)}$ is given by  
\[
\bkappa^{(i)}(\bx,\bomega) \approx \ba_0^{(i)}(\bx) + \sum_{l=1}^{d^{(i)}} \sqrt{\lambda_l^{(i)}}\psi_l^{(i)}(\bx) \bxi_l^{(i)}(\bomega)\,,
\quad \bx\in \mathcal{D}^{(i)}\,.
\]
\end{definition}
Given global random variables $\{\bxi_j\}_{j=1}^d$, the link of the local random variable and the global random variables can be found as  
\begin{align}
    \bxi_l^{(i)}(\bomega) 
    & = \frac{1}{\sqrt{\lambda_l^{(i)}}} \int_{\calD^{(i)}} [\ba^{(i)}(\bx,\bxi^{(i)}(\bomega)) - \ba_0^{(i)}(\bx)] \psi_l^{(i)}(\bx) \dif \bx\nonumber\\
    & = \frac{1}{\sqrt{\lambda_l^{(i)}}} \int_{\calD^{(i)}} [\ba(\bx,\bxi(\bomega)) - \ba_0(\bx)] \psi_l^{(i)}(\bx) \dif \bx\nonumber\\
    & \approx \frac{1}{\sqrt{\lambda_l^{(i)}}} \sum_{j=1}^d \sqrt{\lambda_j}\bxi_j(\bomega)\int_{\calD^{(i)}} \psi_j(\bx) \psi_l^{(i)}(\bx)\dif \bx\,.\nonumber %\label{eq:link_local_global}\,.
\end{align}
Here we extend the definition of local eigenfunctions to the global domain 
\[
\forall \bx\in \calD\,,\quad 
\widetilde{\psi}_j^{(i)}(\bx) = 
\begin{cases}
\psi_j^{(i)}(\bx) \,,\quad \bx \in \calD^{(i)}\,,\\
0\,,\quad \text{otherwise}\,.
\end{cases}
\]
By compensating the definition in $(\calD^{(i)})^c:=\calD/\calD^{(i)}$ for $i=1,\ldots,M$, the collected sets of eigenfunctions $\{\psi_j^{(i)}(\bx)\}_{j=1,\ldots,\infty, i=1,\ldots,M}$ can form an orthonormal basis of $L_2(\calD)$.
In that way, the resulting random field is well defined over the global domain $\calD$, i.e., for $\bx\in \calD$, 
\begin{equation}
\label{eq:local_field}
\widetilde{\bkappa}^{(i)}(\bx,\bomega) \approx\widetilde{\ba}^{(i)}(\bx,\bxi^{(i)}(\bomega)):=
\begin{cases}
\ba_0^{(i)}(\bx) + \sum_{j=1}^{d^{(i)}}\sqrt{\lambda_j^{(i)}}\psi_j^{(i)}(\bx)\bxi_j^{(i)}(\bomega)\,,\quad \bx \in \calD^{(i)}\,,\\
0\,,\quad \text{otherwise}\,.
\end{cases}
\end{equation}

Accordingly, the \textit{local forward model} is defined as
\[
\bd^{(i)} = \bF^{(i)}(\ba^{(i)}(\bx,\bxi^{(i)}(\bomega))+\bepsilon^{(i)}\,.
\]
%Assume the local KLE for the local field is
Consequently, we can define the \textit{stitched} global random field by directly combining the local patches together.

\begin{definition}[The stitched random filed]
The stitched random field is defined as the collection of the random fields over subdomains,
\[
\breve{\ba}(\bx,\bxi(\bomega)) = \sum_{i=1}^M \widetilde{\ba}^{(i)}(\bx,\bxi(\bomega))\,,\quad
\bx\in \calD\,,
\]
where $\widetilde{\ba}^{(i)}$ is defined in \eqref{eq:local_field}.
\end{definition}

The local random variables $\{ \bxi^{(i)}(\bomega)\}_{i=1}^M$ follows the same distribution as the global random field, i.e., if the global random field is Gaussian, then the restriction operator does not change the Gaussian property of the local random field.

\iffalse
\textcolor{red}{
Suppose we are specified the prior distribution for $\bxi$ in the global domain, now the problem is, what is the distribution of local parameters $\bxi_j^{(i)}$?
Write \eqref{eq:local_para} further, for $j=1,\ldots, d^{(i)}$,
\begin{align}
    	\bxi_j^{(i)}  
    	 & = \frac{1}{\sqrt{\lambda_j^{(i)}}} \int_{\calD^{(i)}} [\ba^{(i)}(\bx,\bxi) - \ba_0^{(i)}(\bx)] \psi_j^{(i)}(\bx) \dif \bx \nonumber\\
    	 & = \frac{1}{\sqrt{\lambda_j^{(i)}}} \int_{\calD^{(i)}} \left[\sum_{l=1}^{d} \sqrt{\lambda_l} \bxi_l \psi_l(\bx)\right] \psi_j^{(i)}(\bx) \dif \bx \nonumber\\
    	 & = \frac{1}{\sqrt{\lambda_j^{(i)}}} \sum_{l=1}^{d} \sqrt{\lambda_l}\bxi_l \int_{\calD^{(i)}} \psi_l(\bx)\psi_j^{(i)}(\bx)\dif \bx\,,
    	 \label{eq:decompose_rv}
\end{align}
for fixed subdomain $\calD^{(i)}$, we can see that $\bxi_j^{(i)}$ is a linear combination of a set of independent random variables $\{\bxi_l\}_{l=1}^{\infty}$.
Throughout this paper, we assume that the prior distribution of $\{\bxi_l\}$ is standard Gaussian, 
by Cauchy-Schwarz inequality, we have that
\begin{align*}
& \left(\int_{\calD^{(i)}}\psi_l(\bx) \psi_j^{(i)}(\bx)\dif \bx\right)^2 \le \left(\int_{\calD^{(i)}}\psi_l^2(\bx) \dif \bx \right)
\left( \int_{\calD^{(i)}} (\psi_j^{(i)}(\bx))^2 \dif \bx \right)\\
& \quad  \le \left(\int_{\calD^{(i)}}\psi_l^2(\bx) \dif \bx \right) \le 
\left(\int_{\calD}\psi_l^2(\bx) \dif \bx \right) = 1\,,
\end{align*}
then $\bxi_j^{(i)}$ are also Gaussian with mean 
\begin{align*}
& \mathbb{E}[\bxi_j^{(i)}] = 0\,, \\
& \mathbb{V}[\bxi_j^{(i)}] = \sum_{l=1}^{\infty} \left( \sqrt{\frac{\lambda_l}{\lambda_j^{(i)}}} \int_{\calD^{(i)}} \psi_l(\bx) \psi_j^{(i)}(\bx)\dif x \right)^2 \le 
\sum_{l=1}^{\infty} \frac{\lambda_{l}}{\lambda_j^{(i)}} 
\end{align*}
where we can see that 
$
\sum_{l=1}^{\infty} \frac{\lambda_{l}}{\lambda_j^{(i)}}  
$ is greater than 1 since $\lambda_j > \lambda_j^{(i)}$. Therefore, the variance of the prior distribution increases.
Numerical experiments show that the local random variables follow the same distribution with the global random variables.}
\fi

As \cite{chen2015local} pointed out, the decay rate of the eigenvalues depends on the relative correlation length other than the correlation length of the covariance function.
To be more specific, consider the random process $\ba(\bx,\bxi(\bomega))$ with a correlation length $\ell_a$ in a physical domain $E$, then its relative correlation length $\ell_{a,E}$ satisfies 
\[
\ell_{a,E} \propto \ell_a /\ell_{E}\,,
\]
where $\ell_E$ scales as the diameter of the domain $E$. 
The eigenvalues are positive and nonincreasing. As long as the correlation of the process is nonzero, the eigenvalues will decrease. 
Typically, the longer the correlation length, the faster the decay, and vice versa.

Also, we remark that the reduction in dimension is due to domain decomposition.
The use of subdomains introduces no addition error into the parameterization since the transformation from the global random field to the local random field is achieved via restriction.

\subsection{Assembled KL expansion}
Direct construction of the global parameter field from local parameters and then stitching all subdomains together is likely to produce fields with rough boundaries. 
We, therefore, add a post-processing step that finds the best matching global KL expansion reconstruction. 
Moreover, we restrict our discussion with a deterministic perspective since the step is \textit{post-processing}. 

%Consider one sample $\bxi(\bomega)$ of the global field $\ba(\bx,\bxi(\bomega))$, which is referred to as the reference field in the sequel.
%Then, in the forward sense, local variables $\bxi^{(i)}(\bomega)$ of the local domain $\calD^{(i)}$ can be computed from the global variable $\bxi(\bomega)$.
%Inversely, 
Suppose a sequence of local parameters $\bxi^{(i)}_l(\bomega), i=1,\ldots,M, l=1,\ldots, d^{(i)}$ are at hand, then the global variable can be assembled as 
\begin{equation}
	\widehat{\bxi}_j(\bomega) = \frac{1}{\sqrt{\lambda_j}}\sum_{i=1}^M\sum_{l=1}^{d^{(i)}}\sqrt{\lambda_l^{(i)}}\bxi_l^{(i)}(\bomega)\int_{\calD^{(i)}} \psi_l^{(i)}(\bx)\psi_j(\bx)\dif \bx\,,\quad j =1,\ldots,d\,.
	\label{eq:assemble_rv}
\end{equation}
Denoting the resulting assembled KL variables as $\widehat{\bxi}(\bomega) = [\widehat{\bxi}_1(\bomega),\ldots,\widehat{\bxi}_d(\bomega)]$, we can define the assembled field as follows.

\begin{definition}[The assembled filed]
\label{def:assembled_field}
Given a set of local variables $\{\bxi^{(i)}(\bomega)\}_{i=1}^M$, the assembled field is given by 
\begin{equation}
\label{eq:assembled_kle}
    \widehat{\ba}(\bx,\widehat{\bxi}(\bomega)) = \ba_0(\bx) + \sum_{j=1}^d \sqrt{\lambda_j} \psi_j(\bx)\widehat{\bxi}_j(\bomega)\,, 
\end{equation}
where $\{\widehat{\bxi}_j(\bomega)\}_{j=1}^{d}$ are defined in \eqref{eq:assemble_rv}, the mean function and the eigenpairs follow the same setting in \eqref{eq:kle_inf}.
\end{definition}

%Consider one realization $\bomega$ of local random fields $\{\ba^{(i),\infty}(\bx,\bxi^{(i)}(\bomega))\}_{i=1}^M$, the random variables of the global random field can be reconstructed in the way that, for $j=1,\ldots,d$,
%\begin{align*}
%	\bxi_j(\bomega) 
%	& = \frac{1}{\sqrt{\lambda_j}} \int_\calD [\ba^{\infty}(\bx,\bx(\bomega)) - \ba_0(\bx)] \psi_j(\bx) \dif \bx\\ 
%	& = \frac{1}{\sqrt{\lambda_j}} \int_{\cup_{i=1}^M \calD^{(i)}}[\ba^{\infty}(\bx,\bxi(\bomega)) - \ba_0(\bx)] \psi_j(\bx) \dif \bx \\
%	& = \frac{1}{\sqrt{\lambda_j}} \sum_{i=1}^M \int_{\calD^{(i)}}[\ba^{\infty}(\bx,\bxi(\bomega)) - \ba_0(\bx)] \psi_j(\bx) \dif \bx\\
%	& = \frac{1}{\sqrt{\lambda_j}} \sum_{i=1}^M \int_{\calD^{(i)}}[\ba^{\infty}(\bx,\bxi(\bomega)) - \ba_0(\bx)]\mathbb{I}_{\calD^{(i)}}(\bx) \psi_j(\bx) \dif \bx\\
%	& 
%	= \frac{1}{\sqrt{\lambda_j}} \sum_{i=1}^M \int_{\calD^{(i)}}[\ba^{(i),\infty}(\bx,\bxi(\bomega)) - \ba_0^{(i)}(\bx)] \psi_j(\bx) \dif \bx \\
%	& = \frac{1}{\sqrt{\lambda_j}} \sum_{i=1}^M \int_{
%\calD^{(i)}}\left[\sum_{l=1}^{+\infty} \sqrt{\lambda_l^{(i)}} \psi_l^{(i)}(\bx)\bxi_l^{(i)}(\bomega)\right] \psi_j(\bx) \dif \bx\\
%	&= \frac{1}{\sqrt{\lambda_j}}\sum_{i=1}^M\sum_{l=1}^{+\infty}\sqrt{\lambda_l^{(i)}}\bxi_l^{(i)}(\bomega)\int_{\calD^{(i)}} \psi_l^{(i)}(\bx)\psi_j(\bx)\dif \bx\\
%	& \approx \frac{1}{\sqrt{\lambda_j}}\sum_{i=1}^M\sum_{l=1}^{d^{(i)}}\sqrt{\lambda_l^{(i)}}\bxi_l^{(i)}(\bomega)\int_{\calD^{(i)}} \psi_l^{(i)}(\bx)\psi_j(\bx)\dif \bx=: \widehat{\bxi}_j(\bomega) \,.
%\end{align*}
% Now considering a global field $\ba(\bx,\bxi(\bomega))$ which is referred to as the reference filed in the sequel, let the $\{\bxi^{(i)}(\bomega)\}_{i=1}^{M}$ be the corresponding local parameters.
% We can show that the approximation error of the assembled field compared to the reference filed is mainly induced by truncation error.
%\begin{proposition}
%The approximation error of the assembled field towards the reference field is bounded and finite,
%\[
%\|\widehat{\ba}(\bx,\widehat{\bxi}(\bomega)) - \ba(\bx,\bxi(\bomega)) \|_{\calD}^2\le d \sum_{i=1}^{M}\sum_{l=d^{(i)}+1}^{+\infty}\lambda_l^{(i)}(\bxi_l^{(i)}(\bomega))^2\,,
%\]
%where $\widehat{\ba}(\bx,\widehat{\bxi}(\bomega))$ is given in Definition \ref{def:assembled_field}.
% \end{proposition}

% \begin{proof}
%For $j=1,\ldots,d$,
%\begin{align*}
%e_j: = \bxi_j(\bomega) - \widehat{\bxi}_j(\bomega)
%     & = \frac{1}{\sqrt{\lambda_j}}\sum_{i=1}^M\sum_{l = d^{(i)}+1}^{+\infty}\sqrt{\lambda_l^{(i)}}\bxi_l^{(i)}(\bomega)\int_{\calD^{(i)}} \psi_l^{(i)}(\bx)\psi_j(\bx)\dif \bx \\
%     & \le \frac{1}{\sqrt{\lambda_j}}\sum_{i=1}^M\sum_{l = d^{(i)}+1}^{+\infty}\sqrt{\lambda_l^{(i)}}\bxi_l^{(i)}(\bomega)
%     \,,
%\end{align*}
%where 
%\begin{align*}
%    & \left(\int_{\calD^{(i)}} \psi_l^{(i)}(\bx)\psi_j(\bx)\dif \bx \right)^2 \le 
%    \left( \int_{\calD^{(i)}} (\psi_l^{(i)})^2(\bx) \dif \bx  \right)\left( \int_{\calD^{(i)}} \psi_j^2(\bx) \dif \bx  \right)\\
%    &\quad \le \left( \int_{\calD^{(i)}} (\psi_l^{(i)})^2(\bx) \dif \bx  \right)\left( \int_{\calD} \psi_j^2(\bx) \dif \bx  \right)=1\,,
        %\le \int_{\calD^{(i)}} \psi_l^{(i)}^2(\bx)\dif \bx \le 
%\end{align*}
% then,
%\begin{align}
%    & \| \widehat{\ba}(\bx,\widehat{\bxi}(\bomega) - \ba(\bx,\bxi(\bomega)) \|_{\calD}^2 = \left\|
%    \sum_{j=1}^d\sqrt{\lambda_j}\psi_j(\bx)\underbrace{\widehat{\bxi}_j(\bomega) - \bxi_j(\bomega) )}_{e_j}\right\|_{\calD}^2 \nonumber\\
%    &\quad \le \sum_{j=1}^d\left\| \sqrt{\lambda_j}\psi_j(\bx)e_j\right\|_{\calD}^2 = \sum_{j=1}^d \int_{\calD}\lambda_j e_j^2 \psi_j(\bx)^2 \dif \bx = \sum_{j=1}^d\lambda_j e_j^2 \nonumber \\
%    & \quad \le d \left(\sum_{i=1}^M \sum_{l=d^{(i)}+1}^{+\infty}\sqrt{\lambda_l^{(i)}}\bxi_l^{(i)}(\bomega) \right)^2 \le 
%    d \sum_{i=1}^M \sum_{l=d^{(i)}+1}^{+\infty}\lambda_l^{(i)}(\bxi_l^{(i)}(\bomega))^2\,.
%    \label{eq:field_error}
% \end{align}
% \end{proof}
%Therefore, we can see that the error is dominated by the truncation error of local KL expansion and is finite.
%By increasing the number of terms in local KL expansion, we can control the error.

\begin{theorem}
The centralized assembled field $\widehat{\ba}(\bx,\widehat{\bxi}(\bomega))-\ba_0(\bx)$ is the projection of the centralized stitched field $\breve{\ba}(\bx,\bxi(\bomega)) - \ba_0(\bx)$
%$\sum_{i=1}^M [\widetilde{\ba}^{(i)}(\bx,\bxi^{(i)}(\bomega)) - \ba_0^{(i)}(\bx)]$ 
onto the subspace spanned by global eigenfunctions $\{\psi_i(\bx)\}_{i=1}^d$.
\end{theorem}

\begin{proof}
We denote the projection of a vector $\mathbf{vec}$ onto the subspace $\mathbb{V}$ as $\mathbf{vec}_{\mathbb{V}}$.
Take $\mathbb{V}_1$ as the space spanned by $\{\psi_j(\bx):j=1\ldots,d\},$ $\mathbb{V}_2$ as the space spanned by 
$\{\widetilde{\psi}_l^{(i)}(\bx):i=1,\ldots,M, l=1,\ldots,d^{(i)}\}$,
then we can see that the $\widehat{\ba}(\bx,\bxi(\bomega)) - \ba_0(\bx)\in \mathbb{V}_1$ and $\breve{\ba}(\bx,\bxi(\bomega))-\ba_0(\bx) \in \mathbb{V}_2 $.
%the centralized field $[\ba(\bx,\bxi(\bomega)) - \ba_0(\bx)]= \sum_{j=1}^d \sqrt{\lambda_j}\psi_j(\bx)\bxi_j\in \mathbb{V}_1$, and its projection onto $\mathbb{V}_2$ is given by taking its inner products of the basis of $\mathbb{V}_2$, 
%\begin{align*}
%    &[\ba(\bx,\bxi(\bomega)) - \ba_0(\bx)]_{\mathbb{V}_2}
%    = \sum_{i=1}^M \sum_{l=1}^{d^{(i)}} \langle
%\ba(\bx,\bxi(\bomega)) - \ba_0(\bx), \widetilde{\psi}_l^{(i)}(\bx)\rangle\widetilde{\psi}_l^{(i)}(\bx)\\
%&\quad = \sum_{j=1}^{d} \sqrt{\lambda_j}\bxi_j(\bomega) \sum_{i=1}^M \sum_{l=1}^{d^{(i)}} \langle \widetilde{\psi}_l^{(i)}(\bx), \psi_j(\bx) \rangle \widetilde{\psi}_l^{(i)}(\bx)\,,
%\end{align*}
%which is exactly the centralized stitched field. 
%We can see this in 
%\begin{align*}
    %&\sum_{i=1}^M \widetilde{\ba}^{(i)}(\bx,\bxi(\bomega)) - \ba_0(\bx)  =
%    &\sum_{i=1}^M [\widetilde{\ba}^{(i)}(\bx,\bxi(\bomega)) - \ba_0^{(i)}(\bx)] = \sum_{i=1}^M \sum_{l=1}^{d^{(i)}} \bxi_l^{(i)}(\bomega)\sqrt{\lambda_l^{(i)}}\widetilde{\psi}_l^{(i)}(\bx)\\
%    &\quad = \sum_{i=1}^M \sum_{l=1}^{d^{(i)}} \frac{1}{\sqrt{\lambda_l^{(i)}}}\sum_{j=1}^d \sqrt{\lambda_j}\bxi_j(\bomega) \int_{\calD^{(i)}}\psi_j(\bx)\widetilde{\psi}_l^{(i)}\dif \bx  \sqrt{\lambda_l^{(i)}}\widetilde{\psi}_l^{(i)}(\bx)\\
%    &\quad  =\sum_{j=1}^{d} \sqrt{\lambda_j}\bxi_j(\bomega) \sum_{i=1}^M \sum_{l=1}^{d^{(i)}} \langle \widetilde{\psi}_l^{(i)}(\bx), \psi_j(\bx) \rangle \widetilde{\psi}_l^{(i)}(\bx) = [\ba(\bx,\bxi(\bomega)) - \ba_0(\bx)]_{\mathbb{V}_2}\,.
%\end{align*}
Rewrite the centralized assembled field
\begin{align*}
    &\widehat{\ba}(\bx,\widehat{\bxi}(\bomega)) - \ba_0(\bx)  
     =\sum_{j=1}^d \sqrt{\lambda_j}\psi_j(\bx) \widehat{\bxi}_j(\bomega)\\ 
    &\quad  = \sum_{j=1}^d  \sqrt{\lambda_j}\psi_j(\bx) \frac{1}{\sqrt{\lambda_j}}\sum_{i=1}^M\sum_{l=1}^{d^{(i)}}\sqrt{\lambda_j^{(i)}}\bxi_l^{(i)}(\bomega)\int_{\calD^{(i)}} \widetilde{\psi}_l^{(i)}(\bx)\psi_j(\bx)\dif \bx \\
    %& \quad = \sum_{j=1}^d \left(\sum_{i=1}^M\sum_{l=1}^{d^{(i)}}\sqrt{\lambda_j^{(i)}}\bxi_l^{(i)}(\bomega) \int_{\calD^{(i)}}\widetilde{\psi}_l^{(i)}(\bx)  \psi_j(\bx)\dif \bx\right)\psi_j(\bx)\\
    & \quad = \sum_{j=1}^d \sum_{i=1}^M\sum_{l=1}^{d^{(i)}}\sqrt{\lambda_j^{(i)}}\bxi_l^{(i)}(\bomega)\langle\widetilde{\psi}_l^{(i)}, \psi_j\rangle_{\calD^{(i)}} \psi_j(\bx) \\
    % &\quad= \sum_{j=1}^d \left\langle
    % \sum_{i=1}^M \sum_{l=1}^{d^{(i)}}\sqrt{\lambda_l^{(i)}} \bxi_l^{(i)}(\bomega)\widetilde{\psi}_l^{(i)}(\bx), \psi_j(\bx) \right\rangle_{\calD^{(i)}} \psi_j(\bx)\\
    & \quad =\sum_{j=1}^d \left\langle
    \sum_{i=1}^M [\widetilde{\ba}^{(i)}(\bx,\bxi^{(i)}(\bomega)) - \ba_0^{(i)}(\bx)],\psi_j(\bx)\right\rangle_{\calD^{(i)}} \psi_j(\bx) \\
    & \quad =\sum_{j=1}^d \left\langle
    \breve{\ba}(\bx,\bxi(\bomega)) - \ba_0(\bx),\psi_j(\bx)\right\rangle_{\calD^{(i)}} \psi_j(\bx) 
    \,. 
\end{align*}
Therefore the centralized assemble field can be seen as the projection of \textit{stitched field} $[\breve{\ba}(\bx,\bxi(\bomega)) - \ba_0(\bx)]$ onto the subspace $\mathbb{V}_1$.
\end{proof}
For arbitrary basis function $\psi_n(\bx)$ of $\mathbb{V}_1$, $n=1,\ldots,d$, 
\begin{align*}
    & \langle \widehat{\ba}(\bx,\bxi(\bomega)) - \breve{\ba}(\bx,\bxi(\bomega)),\psi_n\rangle_{\calD} \\
    & = 
    \left\langle \sum_{j=1}^d \langle
    \breve{\ba}(\bx,\bxi(\bomega)) - \ba_0(\bx),\psi_j\rangle_{\calD^{(i)}}\psi_j + \ba_0(\bx) -  \breve{\ba}(\bx,\bxi(\bomega))
    ,\psi_n\right\rangle_{\calD}\\
    & = \sum_{j=1}^d \langle
    \breve{\ba}(\bx,\bxi(\bomega)) - \ba_0(\bx),\psi_j\rangle_{\calD^{(i)}} \langle \psi_j
    ,\psi_n\rangle_{\calD}
    - 
    \langle \breve{\ba}(\bx,\bxi(\bomega)) - \ba_0(\bx)
    ,\psi_n\rangle_{\calD} =0 \,,
\end{align*}
we can see that $(\widehat{\ba}- \breve{\ba}) \perp \mathbb{V}_1$.
Therefore for any $\ba(\bx,\bxi(\bomega))\in \mathbb{V}_1$, we have 
\begin{align*}
    & \| \ba(\bx,\bxi(\bomega)) -\breve{\ba}(\bx,\bxi(\bomega)) \|_{\calD} =\| \ba(\bx,\bxi) - \widehat{\ba}(\bx,\bxi(\bomega)) + \widehat{\ba}(\bx,\bxi(\bomega))-  \breve{\ba}(\bx,\bxi(\bomega))  \|_{\calD} \\
    &\quad = 
    \| \ba(\bx,\bxi(\bomega)) - \widehat{\ba}(\bx,\bxi(\bomega)) \|_{\calD}+ \|\widehat{\ba}(\bx,\bxi(\bomega))-  \breve{\ba}(\bx,\bxi(\bomega))  \|_{\calD}\,,
\end{align*}
consequently, $\|\ba(\bx,\bxi(\bomega)) -\widehat{\ba}(\bx,\bxi(\bomega)) \|_{\calD} \le \| \ba(\bx,\bxi(\bomega)) -\breve{\ba}(\bx,\bxi(\bomega)) \|_{\calD}$.
In Figure. \ref{fig:random_field_reconstruction}, we show the comparison of the stitched field $\breve{\ba}$ and the assembled field $\widehat{\ba}$.  
\begin{figure}
\centering
%\subfigure{
%      \includegraphics[scale=0.3]{Figures/KLE/global_kle.eps}
%      \label{fig:global_kle}
%      }
\subfigure{
      \includegraphics[scale=0.3]{Figures/KLE/stitched_kle.eps}
      \label{fig:stitched_kle}
      }
\subfigure{
      \includegraphics[scale=0.3]{Figures/KLE/assembled_kle.eps}
      \label{fig:assembled_kle}
      }
      \caption{Comparison of the stitched field and the assembled field}
\label{fig:random_field_reconstruction}
\end{figure}

\section{Domain-Decomposed Markov chain Monte Carlo (DD-MCMC)}
In this section, we demonstrate our Domain-Decomposed Markov chain Monte Carlo (DD-MCMC) algorithm.

\subsection{Guassian process for interface treatment}
Let the complete data set over the global domain be $\bS = \{ (\bx^{j}, \bd^{j})\}_{j=1}^n$ and $\bS^{(i)} = \{ (\bx^{(i),j}, \bd^{(i),j})\}_{j=1}^{n^{(i)}}$ the data restricted in subdomain $\calD^{(i)}$.
In addition, denote the data on the interface $\btau^{(i,j)}$ as $\bS^{(i,j)}$. 
%If the data is not collected on the interface, then $\bS^{(i,j)}=\emptyset$.
After domain decomposition, 
even though the dimension of the unknown parameter is drastically reduced, the interface condition is exposed as unknown. 
In the area of domain decomposition, the unknown interface condition can be a daunting issue, and iterative methods such as the Schwarz alternating method are used to update the boundary condition \cite{xu1998some, quarteroni1999domain}. 
However, in the inverse setting, we have access to data near or on the interface, which can be used to do data regression in order to construct a sufficiently accurate Dirichelt condition for the interface \cite{jagtap2020conservative, shukla2021parallel}.

Consequently, many regression methods can be utilized for this data regression task.
Here we use the Gaussian process \cite{rasmussen2003gaussian, kennedy2001bayesian, oakley2002bayesian, kennedy2006case} to simulate the interface condition for two reasons.
First, Gaussian process regression
is a widely used emulating technique \cite{chen2020anova,bilionis2013multi, atkinson2019structured, wang2018adaptive}, especially for 
such a relatively low dimensional case.
Second, since the data we have is partial, the interface condition we predict is not accurate, the Gaussian process can simulate the uncertainty within. 
We denote $\bLambda^{(i,j)}$ the training data used for fitting the interface $\btau^{(i,j)}$ and $n^{(i,j)} := |\bLambda^{(i,j)}|$ denotes its size.
%and for the notation of simplicity, we denote $\bS^{(i,j)}$ the data restricted either on the interface of subdomains $\calD^{(i)}$ and $\calD^{(j)}$ or near the interface, i.e., $\bS^{(i,j)} = \{ \bx^l,l=1\ldots, n^{(i,j)}| \bx^{l} \in \btau^{(i,j)}\}$.
To avoid any confusion in notation, we use $h^{(i,j)}(\bx)$ to denote the mapping from physical location to its PDE solution on the interface $\btau^{(i,j) }$, specifically, $h^{(i,j)}(\bx)=u(\bx)$ when $\bx \in \btau^{(i,j)}$. 

Gaussian process puts a prior over the target function $h^{(i,j)}(\bx)$, which is completely characterized by its mean function $\mu(\bx)$ and kernel function $k(\bx,\bx')$, i.e.,
$h^{(i,j)}(\bx) \sim \mathcal{GP}(\mu(\bx), k(\bx, \bx'))$. Having collected noisy data, GP can provide a posterior distribution for arbitrary point on the interface $\bx^{\star}\in \btau^{(i,j)}$,
\begin{equation}
\label{eq:gp_post}
h^{(i,j)}(\bx^\star)|\bS^{(i,j)}, \bx^{\star} \sim
\widetilde{h}^{(i,j)}:=\mathcal{N}(\mu_{n^{(i,j)}}(\bx^{\star}), \sigma_{n^{(i,j)}}(\bx^{\star}))\,,
\end{equation}
with mean function $\mu_{n^{(i,j)}}(\bx^{\star})$ and variance function $\sigma_{n^{(i,j)}}(\bx^{\star})$ given by 
\begin{align*}
	& \mu_{n^{(i,j)}}(\bx^{\star}) = k_{n^{(i,j)}}(\bx^{\star})^T (K_{n^{(i,j)}} + \bSigma)^{-1}h_{n^{(i,j)}}(\bx^{\star})\,,\\
	& \sigma_{n^{(i,j)}}(\bx^{\star}) = K(\bx^{\star}, \bx^{\star}) - k_{n^{(i,j)}}(\bx^{\star})^T (K_{n^{(i,j)}} + \bSigma)^{-1}k_{n^{(i,j)}}(\bx^{\star})\,,
\end{align*}
where 
\begin{align*}
	& k_{n^{(i,j)}}(\bx^{\star}) = [k(\bx^{\star}, \bx^l)]_{n^{(i,j)}\times 1}\,, 
	\quad K_{n^{(i,j)}} = [k(\bx^l, \bx^{l'})]_{n^{(i,j)} \times n^{(i,j)}},\\
	& h_{n^{(i,j)}}(\bx) = [h^{(i,j)}(\bx^l)]_{n^{(i,j)}\times 1}\,.
\end{align*}
In this work, the kernel function we use is the Gaussian kernel, also known as the squared exponential kernel, i.e., $k(\bx,\bx') = \sigma_f^2 \exp(-\|\bx - \bx'\|_2^2/(2l_f^2)$, where the signal variance $\sigma_f$ and the length-scale $l_f$ are both hyperparameters of the kernel function.
Denoting $\gamma = [\sigma_f, l_f]$ as a vector containing all the hyperparameters, the hyperparameters can be determined from training data through minimizing the negative log marginal likelihood $\mathcal{M}(\gamma):= -\log p(\bS^{(i,j)}|\gamma)$  \cite[Chapter 5.4]{rasmussen2003gaussian}.
%We denote the posterior mean function for $\widetilde{h}^{(i,j)}(\bx)$ as $\bar{h}^{(i,j)}(\bx)$ and the variance function as $\sigma^{(i,j)}(\bx)$.

Utilizing the posterior mean function for the boundary, the altered parameterized forward sub-problem with GP-fitted interface is then defined as 
\begin{equation}
\label{eq:sub_problem_gp_boundary}
\begin{aligned}
	&\mathcal{L}^{(i)} (\bx,u^{(i)};\ba^{(i)}(\bx,\bxi(\bomega))) = f(\bx,\ba^{(i)})\,,\quad \bx\in \calD^{(i)}\,, \\
	&\mathcal{B}^{(i)}(\bx, u^{(i)};\ba^{(i)}(\bx,\bxi(\bomega))) = g^{(i)}(\bx,\ba)\,,\quad \bx\in \partial \calD^{(i)}\cap \partial \calD\,,\\
	& \mathcal{B}^{(i,j)} (\bx, u^{(i)}; \ba^{(i)}(\bx,\bxi(\bomega))) =
	\widetilde{g}_{\text{GP}}^{(i,j)}(\bx,\ba)\,,\quad \bx \in \btau^{(i,j)}\,,\quad j \ne i\,,
\end{aligned}
\end{equation}
where $\widetilde{g}_{\text{GP}}^{(i,j)}(\bx,\ba)=\mu_{n^{(i,j)}}(\bx)$ encodes the GP-fitting interface condition.
Denoting the \textit{local GP-fitting interface} forward PDE model as $\bF_{\text{GP}}^{(i)}$, we can see that, compared to the forward model with exact interface condition \eqref{eq:sub_problem}, the GP-fitting interface condition inserts additive error to the forward mapping, 
\[
\bd^{(i)} = \bF^{(i)}(\ba^{(i)}(\bx^{(i)},\bxi(\bomega))) +\bepsilon^{(i)} = 
\bF^{(i)}_{\text{GP}}(\ba^{(i)}(\bx^{(i)},\bxi(\bomega))) + \bm{\zeta}^{(i)} +\bepsilon^{(i)}\,,
\]
where the model error $\bm{\zeta}^{(i)}:= \bF^{(i)}(\ba^{(i)}(\bx^{(i)},\bxi(\bomega)))  \bF^{(i)}_{\text{GP}}(\ba^{(i)}(\bx^{(i)},\bxi(\bomega)))$ describes the effects of partial uncertain interface conditions.
However, $\bm{\zeta}^{(i)}$ is relatively small and also hard to quantify, therefore we define the following \textit{reduced local} forward model,
\[
\widetilde{\bd}_\text{GP}^{(i)} =
\widetilde{\bF}^{(i)}_{\text{GP}}(
\ba^{(i)}(\bx^{(i)}, \bxi^{(i)}(\bomega))) +\bepsilon^{(i)}\,.
\]
As \cite{cui2015data} remark, the samples drawn from an approximate posterior distribution, the resulting Monte Carlo estimator based on the approximate posterior samples is biased. 
%The global forward model resides in the global high-dimensional parameter space, on the contrary, we refer \eqref{eq:local_forward} to as the \textit{local} forward model with exact boundary condition.

We use $\mathcal{K}(\bx^i, \bx^j)$ to denote the standard Euclidean distance between two data points in $\mathcal{D}$, i.e., $\mathcal{K}(\bx^i, \bx^j):=\|\bx^i - \bx^j\|_2$.
Consequently, 
considering the interface $\btau^{(i,j)}$,
the Euclidean distance of one data point to the interface is defined as the shortest distance of the data point to any point of the interface, i.e.,  $\mathcal{K}(\bx^r,\btau^{(i,j)}):=\min_{\bx^r, \bx^j\in\btau^{(i,j)}}\mathcal{K}(\bx^r, \bx^j)$. 
Moreover, define $\bS^{(i,j),\epsilon}$ containing all the training data whose distance towards the interface $\btau^{(i,j)}$ is less than $\epsilon$, 
\[
\bS^{(i,j),\epsilon}:= \{ (\bx^r,\bd^r)\in\bS|\, \mathcal{K}(\bx^r, \btau^{(i,j)})\le \epsilon \}\,.
\]
Suppose the spatial discretization on the interface $\btau^{(i,j)}$ is carried out on a $N^{(i,j)}$-element mesh, $\Delta^{(i,j)}:=\{\bx^{r}, r=1,\ldots,N^{(i,j)}|\bx^r\in\btau^{(i,j)}\}$.
In practice, we can easily letting $\bLambda^{(i,j)}=\bS$ since it in theory maximizes the possible informativeness. However, it can be unnecessary in that the data far away from the interface cannot provide much information. 
Therefore, to improve the efficiency, we consider expanding the training dataset in a \textit{sequential} format when training the GP model.

We initialize the training data set $\bLambda^{(i,j)}$ as containing the data points only on the boundary, i.e., $\bLambda^{(i,j)} = \bS^{(i,j)}$. 
Naturally, the maximum posterior variance of the discretized mesh can serve as an indicator for interface fitting, which is defined as 
\begin{equation}
\label{eq:max_var}
    \sigma_{N^{(i,j)}}^{\max}:=\max_{\bx^r\in \Delta^{(i,j)}}\sigma_{n^{(i,j)}}(\bx^r)\,.
\end{equation}
If the maximum posterior variance reached the pre-set threshold $\delta_{\text{tol}}$, we use the posterior mean function to fit the interface.
Otherwise, we expand the training data $\bLambda^{(i,j)}$ as $\bLambda^{(i,j)}= \bS^{(i,j),\epsilon}$ for the pre-set $\epsilon$, which we refer to as \textit{the expanding distance}.
We present further discussion about the effects of GP-fitting interface in Section \ref{sec:numerical}. 

\subsection{DD-MCMC Algorithm}
So far, given a large-scale inverse problem, we can decompose the problem in a spatial sense and represent the unknown field with local KL random variables. 
A domain-decomposed MCMC algorithm is shown in Algorithm \ref{alg:parallel_MCMC}.
In this algorithm, the interface conditions are fitted using GP and the inversion of each subdomain is performed independently in parallel. 
In each subdomain, the dimension of the unknown parameter is reduced and therefore the application of various sampling methods which have limitations in dimensions are enabled.
Also, this algorithm achieves a reduction in computation cost owing to the parallelization.

% First, a stopping criterion based on the boundary condition is proposed. The initial boundary condition is fitted using the data only restricted within the local domain, and due to this reason, the same boundary shared by two subdomains may have different regression result, 

% \subsection{Globally-informed MCMC method}
% So far, given a large-scale inverse problem, we can decompose the problem in a spatial sense, perform inversion in a parallel manner.
% An vanilla parallel MCMC algorithm without considering communication among local domains is shown in Algorithm. \ref{alg:naive_MCMC}. In this algorithm, the boundary conditions are fitted using GP and the inversion of each subdomain is performed independently. 
% In each subdomain, the dimension of the unknown parameter is reduced and therefore the application of various sampling methods which have limitations in dimensions are enabled.
% Also, this algorithm achieves a reduction in computation cost owing to the parallelization.
% However, this method treats these sub-problems as independent and neglects the implicit relations among local random inputs.
% To exchange information among sub-domains, a globally-informed domain decomposition method is proposed. Take $\bF_C$ be the forward operator over the coarse scale in the global domain and $\bF_F$ be the forward operator over the fine scale in the global domain, and $\bF_F^{(i)}$ denote the forward operator over the fine scale in the $i$-th subdomain.

% Due to uncertain boundary conditions, the local inversion results have larger variance compared to the local problem with accurate boundary conditions.

% In the area of domain decomposition, the information exchange among sub-domains is of crucial importance.
% In the forward computation, the information exchange is achieved via boundary condition iterations. 
% However, in the inverse problems, even though the boundary condition cannot be obtained exactly, we can still give a relatively good initial state using the neighbouring measurements data. 

% First, a stopping criterion based on the boundary condition is proposed. The initial boundary condition is fitted using the data only restricted within the local domain, and due to this reason, the same boundary shared by two subdomains may have different regression result, 

% The globally-informed domain decomposition algorithm we proposed can be easily adjusted to parallelization.

% Communication step among subdomains can greatly slow down the.
% On each subdomain, any classical MCMC method can be used to draw samples from the posterior distribution given the corresponding dataset. 
% Finally, the samples from each subdomain are combined to form samples from the full posterior. 

% The main idea is to borrow the \textit{swap} step to 

\begin{algorithm}[!ht]
    \caption{Domain-Decomposed MCMC method}
    \label{alg:parallel_MCMC}
    \begin{algorithmic}[1]
        \REQUIRE{Dataset $\bS$, global domain $\calD$, covariance function $C(\bx,\by)$, interface threshold $\delta_{\text{tol}}$ and the expanding distance $\epsilon$.}
        \STATE{Partition the global domain $\calD$ into $M$ non-overlapping local domains $\{\calD^{(i)}\}_{i=1}^M$.}
        \STATE{Compute the global KL eigenpairs $\{\lambda_j,\psi_j\}_{j=1}^d$  using \eqref{eq:global_eigenpair}.}
        \STATE{Divide the dataset $\bS$ into $\{\bS^{(i)}\}_{i=1}^M$, $\bS^{(i,j)}$ according to domain division}.
        \FOR{every pair $(i,j)$}{
        \STATE{
        Initialize the training data $\bLambda^{(i,j)}:=\bS^{(i,j)}$, and set $r=1$.}
        \STATE{
        Train the GP model $\widetilde{h}^{(i,j)}:=\mathcal{N}(\mu_{n^{(i,j)}},\sigma_{n^{(i,j)}})$ with $\bLambda^{(i,j)}$ using \eqref{eq:gp_post}}.
        \STATE{Compute the discretized maximum posterior variance $\sigma_{N^{(i,j)}}^{\max}$ using \eqref{eq:max_var}.}
        %Compute the posterior GP mean function $\mu_{N^{(i,j)}}$ and variance function %\sigma_{n^{(i,j)}}$ of $\widetilde{h}^{(i,j)}(\bx)$ for the interface }
        \WHILE{
        $\sigma_{N^{(i,j)}}^{\max}\ge \delta_{\text{tol}}$ and $\bLambda^{(i,j)}\subset \bS$}
        \STATE{Update the training data set as $\bLambda^{(i,j)}=\bS^{(i,j),r\epsilon}$}.
        \STATE{Set $k=k+1$ and go back to line 6.}
        \ENDWHILE
        }
        \STATE{
        Use the posterior mean $\mu_{n^{(i,j)}}$ as the interface condition for $\btau^{(i,j)}$.}
        \ENDFOR
        \STATE{Compute the local KL eigenpairs $\{\lambda_j^{(i)},\psi_j^{(i)}\}_{j=1}^{d^{(i)}}$ for $i=1,\ldots,M$ using  \eqref{eq:local_eigenpair}.} 
        \STATE{Construct the reduced local parameterized forward models $\widetilde{\bF}_{\text{GP}}^{(i)}$ for $i=1,\ldots,M$.}
    %\WHILE{Stopping criteria is satisfied}
    \FOR{ subdomain $i=1,\ldots,M$}
    %\STATE{\textcolor{blue}{$\%$ In a parallel manner}}
    \STATE{Run inversion to obtain posterior samples $\{\bxi^{(i),k}\}_{k=1,\ldots,K^{(i)}}$ with partial data $\bS^{(i)}$ using Algorithm \ref{alg:MHMCMC}.
    (Or other arbitrary sampling methods).}
    \ENDFOR
    %\STATE{\textbf{The SWAP step:} metropolis coupled}
  %\ENDWHILE
  \STATE{Assemble the local inversions to get the assembled random field $\widehat{\ba}$ using \eqref{eq:assembled_kle}.}
  \ENSURE{ The assembled random field $\widehat{\ba}(\bx,\widehat{\bxi}(\bomega)$}.
    \end{algorithmic}
\end{algorithm}

% \begin{algorithm}[!ht]
%    \caption{Globally-informed Metropolis-coupled Parallel MCMC method}
%    \label{alg:gi_MC3}
%    \begin{algorithmic}[1]
%        \STATE{\textbf{Input:} dataset $\bS$, forward local solver $\bF_F^{(i)}$ for $i=1,\ldots,D$, global coarse solver $\bF_C$.}
%        \STATE{Initialization for the boundary conditions.}
%    \FOR{\# Loops}
%    \STATE{Run inversion on \textit{global coarse scale} to obtain $\bxi$ with data $\bS$.}
%    \FOR{subdomain $i=1,\ldots,D$}
%    \STATE{Run inversion to obtain $\bxi^{(i)}$ with partial data $\bS^{(i)}$.}
%    \ENDFOR
%    \STATE{Assemble the local inversions to get the assembled random field $\widehat{\bxi}^{\text{cand}}$ using \eqref{eq:assemble_rv}}
%    \STATE{Decompose inversions to get the local random variables $\widehat{\bxi}^{\text{cand}}$ using \eqref{eq:decompose_rv}}
%    \STATE{\textbf{The SWAP step:} Accept the proposal using a Metropolis step.}
%  \ENDFOR
%  \STATE{Assemble the local inversions to get the assembled random field $\widehat{\ba}$ using \eqref{eq:assembled_kle}.}
%    \end{algorithmic}
% \end{algorithm}

%The algorithm has two parts: \textit{offline} and \textit{online} components.
%In the online stage, various sampling methods can be utilized to perform inversion parallelly and independently. 
%And in the offline stage, forward solvers with boundary fitted by Gaussian process are constructed and the global inversion is given via assembled KLE. 
%The full MCMC does not have an offline stage.



==> Sections/rr_problem_setup_v2.tex <==
\section{Domain-Decomposed Markov chain Monte Carlo (DD-MCMC)}
\label{sec:dd_mcmc}
In this section, we demonstrate our Domain-Decomposed Markov chain Monte Carlo (DD-MCMC) algorithm.

\subsection{Guassian process for interface treatment}
Let $S$ denote the complete data set over the global domain $S := \{ (x^{(s)}, d^{(s)})\}_{s=1}^n$ with size $|S|$.
Also, let $S^{(i)}$ denote the partial data  restricted in subdomain $\calD^{(i)}$ with size $|S^{(i)}|$ for $i=1,\ldots,M$.
In addition, denote the data on the interface $\tau^{(i,j)}$ as $S^{(i,j)}$. 
%If the data is not collected on the interface, then $\bS^{(i,j)}=\emptyset$.
After domain decomposition, 
even though the dimension of the unknown parameter is drastically reduced, the interface condition is exposed as unknown. 
In the area of domain decomposition, the unknown interface condition can be a daunting issue, and iterative methods such as the Schwarz alternating method are used to update the boundary condition \cite{xu1998some, quarteroni1999domain}. 
However, in the inverse setting, we have access to data near or on the interface, which can be used to do data regression in order to construct a sufficiently accurate Dirichelt condition for the interface \cite{jagtap2020conservative, shukla2021parallel}.

Consequently, many regression methods can be utilized for this data regression task.
Here we use the Gaussian process \cite{rasmussen2003gaussian, kennedy2001bayesian, oakley2002bayesian, kennedy2006case} to simulate the interface condition for two reasons.
First, Gaussian process regression
is a widely used emulating technique \cite{chen2020anova,bilionis2013multi, atkinson2019structured, wang2018adaptive}, especially for 
such a relatively low dimensional case.
Second, since the data we have is partial, the interface condition we predict is not accurate, the Gaussian process can simulate the uncertainty within. 
We denote $\Lambda^{(i,j)}=\{(x^{(s)}, d^{(s)})\}_{s=1}^{n^{(i,j)}}$ the training data used for fitting the interface function $g^{(i,j)}$ over $\tau^{(i,j)}$ and $n^{(i,j)} := |\Lambda^{(i,j)}|$ denotes its size.

Gaussian process puts a prior over the target function $g^{(i,j)}(x)$, which is completely characterized by its mean function $\mu(x)$ and kernel function $k(x,x')$, i.e.,
$g^{(i,j)}(x) \sim \mathcal{GP}(\mu(x), k(x, x'))$. Having collected noisy data, GP can provide a posterior distribution for arbitrary point on the interface $x^{\star}\in \tau^{(i,j)}$,
\begin{equation}
\label{eq:gp_post}
g^{(i,j)}(x^\star)|\Lambda^{(i,j)}, x^{\star} \sim
\widetilde{g}^{(i,j)}:=\mathcal{N}(\mu_{n^{(i,j)}}(x^{\star}), \sigma_{n^{(i,j)}}(x^{\star}))\,,
\end{equation}
with the mean function $\mu_{n^{(i,j)}}(x^{\star})$ and the variance function $\sigma_{n^{(i,j)}}(x^{\star})$ given by 
\begin{align*}
	& \mu_{n^{(i,j)}}(x^{\star}) = k_{n^{(i,j)}}(x^{\star})^T (K_{n^{(i,j)}} + \bSigma)^{-1}g_{n^{(i,j)}}(x^{\star})\,,\\
	& \sigma_{n^{(i,j)}}(x^{\star}) = K(x^{\star}, x^{\star}) - k_{n^{(i,j)}}(x^{\star})^T (K_{n^{(i,j)}} + \bSigma)^{-1}k_{n^{(i,j)}}(x^{\star})\,,
\end{align*}
where 
\begin{align*}
	& k_{n^{(i,j)}}(x^{\star}) = [k(x^{\star}, x^{(s)})]_{n^{(i,j)}\times 1}\,, 
	\quad K_{n^{(i,j)}} = [k(x^{(s)}, x^{(s')})]_{n^{(i,j)} \times n^{(i,j)}},\\
	& g_{n^{(i,j)}}(x) = [d^{(s)}]_{n^{(i,j)}\times 1}\,.
\end{align*}
In this work, the kernel function we use is the Gaussian kernel, also known as the squared exponential kernel, i.e., $k(x,x') = \sigma_f^2 \exp(-\|x - x'\|_2^2/(2l_f^2)$, where the signal variance $\sigma_f$ and the length-scale $l_f$ are both hyperparameters of the kernel function.
Denoting $\gamma = [\sigma_f, l_f]$ as a vector containing all the hyperparameters, the hyperparameters can be determined from training data through minimizing the negative log marginal likelihood $\mathcal{M}(\gamma):= -\log p(\Lambda^{(i,j)}|\gamma)$  \cite[Chapter 5.4]{rasmussen2003gaussian}.

We use $\mathcal{K}(x^{(s)}, x^{(s')})$ to denote the standard Euclidean distance between two data points in $\mathcal{D}$, i.e., $\mathcal{K}(x^{(s)}, x^{(s')}):=\|x^{(s)} - x^{(s')}\|_2$.
Consequently, 
considering the interface $\btau^{(i,j)}$,
the Euclidean distance of one data point to the interface is defined as the shortest distance of the data point to any point of the interface, i.e.,  $\mathcal{K}(x^{(s)},\tau^{(i,j)}):=\min_{x^{(s')}\in\tau^{(i,j)}}\mathcal{K}(x^{(s)}, x^{(s')})$. 
Moreover, define $S^{(i,j),\epsilon}$ containing all the training data whose distance towards the interface $\tau^{(i,j)}$ is less than $\epsilon$, 
\[
S^{(i,j),\epsilon}:= \{ (x^{(s)},d^{(s)})\in S|\, \mathcal{K}(x^{(s)}, \tau^{(i,j)})\le \epsilon \}\,.
\]
Suppose the spatial discretization on the interface $\tau^{(i,j)}$ is carried out on a $N^{(i,j)}$-element mesh, $\Delta^{(i,j)}:=\{x^{(s)}, s=1,\ldots,N^{(i,j)}|x^{(s)}\in\tau^{(i,j)}\}$.
In practice, we can easily let $\Lambda^{(i,j)}=S$ since it in theory maximizes the possible informativeness. However, it can be unnecessary in that the data far away from the interface cannot provide much information. 
Therefore, to improve the efficiency, we consider expanding the training dataset in a \textit{sequential} format when training the GP model.

We initialize the training data set $\Lambda^{(i,j)}$ as containing the data points only on the boundary, i.e., $\Lambda^{(i,j)} = S^{(i,j)}$. 
Naturally, the maximum posterior variance of the discretized mesh can serve as an indicator for interface fitting, which is defined as 
\begin{equation}
\label{eq:max_var}
    \sigma_{N^{(i,j)}}^{\max}:=\max_{x^{(s)}\in \Delta^{(i,j)}}\sigma_{n^{(i,j)}}(x^{(s)})\,.
\end{equation}
If the maximum posterior variance reached the pre-set threshold $\delta_{\text{tol}}$, we use the posterior mean function to fit the interface.
Otherwise, we expand the training data $\Lambda^{(i,j)}$ as $\Lambda^{(i,j)}= S^{(i,j),\epsilon}$ for the pre-set $\epsilon$, which we refer to as \textit{the expanding distance}.
We present further discussion about the effects of GP-fitting interface in Section \ref{sec:numerical}.

Utilizing the posterior mean function for the interface, the altered parameterized forward sub-problem with GP-fitted interface is then defined as: find $u^{(i)}(x,\xi): \calD^{(i)}\times I_{\xi^{(i)}}\to \mathbb{R}$ such that  
\begin{equation}
\label{eq:sub_problem_gp_boundary}
\begin{aligned}
	&\mathcal{L}^{(i)} (x,u^{(i)};a^{(i)}(x,\xi^{(i)}(\omega))) = f(x)\,,\quad x\in \calD^{(i)}\,, \\
	&\mathcal{B}^{(i)}(x, u^{(i)};a^{(i)}(x,\xi^{(i)}(\omega))) = g^{(i)}(x)\,,\quad x\in \partial \calD^{(i)}\cap \partial \calD\,,\\
	& \mathcal{B}^{(i,j)} (x, u^{(i)}; a^{(i)}(x,\xi^{(i)}(\omega))) =
	\mu_{n^{(i,j)}}(x)\,,\quad x \in \tau^{(i,j)}\,,\quad j \ne i\,,
\end{aligned}
\end{equation}
where $\mu_{n^{(i,j)}}(x)$ encodes the GP-fitting interface condition.
Denoting the \textit{local GP-fitting interface} forward PDE model as $F_{\text{GP}}^{(i)}(a^{(i)}(x,\xi^{(i)}(\omega)) )$, we can see that, compared to the forward model with exact interface condition \eqref{eq:sub_problem}, the GP-fitting interface condition inserts additive error to the forward mapping, 
\[
d^{(i)} = F^{(i)}(a^{(i)}(x,\xi^{(i)}(\omega))) +\epsilon^{(i)} = 
F^{(i)}_{\text{GP}}(a^{(i)}(x,\xi^{(i)}(\omega))) + \zeta^{(i)} +\bepsilon^{(i)}\,,
\]
where the model error $\zeta^{(i)}:= F^{(i)}(a^{(i)}(x^{(i)},\xi(\omega)))-  F^{(i)}_{\text{GP}}(a^{(i)}(x,\xi^{(i)}(\omega)))$ describes the effects of partial uncertain interface conditions.
However, $\zeta^{(i)}$ is relatively small and also hard to quantify, therefore the local forward model is given by 
\begin{equation}
\label{eq:local_forward_GP}
\widetilde{d}_\text{GP}^{(i)} =
\widetilde{F}^{(i)}_{\text{GP}}(
a^{(i)}(x^{(i)}, \xi^{(i)}(\omega))) +\epsilon^{(i)}\,.
\end{equation}
As \cite{cui2015data} remark, the samples drawn from an approximate posterior distribution, the resulting Monte Carlo estimator based on the approximate posterior samples is biased. 
%The global forward model resides in the global high-dimensional parameter space, on the contrary, we refer \eqref{eq:local_forward} to as the \textit{local} forward model with exact boundary condition.

 

\subsection{DD-MCMC Algorithm}
So far, given a large-scale inverse problem, we can decompose the problem in a spatial sense and represent the unknown field with local KL random variables. 
A domain-decomposed MCMC algorithm is shown in Algorithm \ref{alg:parallel_MCMC}.
In this algorithm, the interface conditions are fitted using GP and the inversion of each subdomain is performed independently in parallel. 
In each subdomain, the dimension of the unknown parameter is reduced and therefore the application of various sampling methods which have limitations in dimensions are enabled.
Also, this algorithm achieves a reduction in computation cost owing to the parallelization.

% First, a stopping criterion based on the boundary condition is proposed. The initial boundary condition is fitted using the data only restricted within the local domain, and due to this reason, the same boundary shared by two subdomains may have different regression result, 

% \subsection{Globally-informed MCMC method}
% So far, given a large-scale inverse problem, we can decompose the problem in a spatial sense, perform inversion in a parallel manner.
% An vanilla parallel MCMC algorithm without considering communication among local domains is shown in Algorithm. \ref{alg:naive_MCMC}. In this algorithm, the boundary conditions are fitted using GP and the inversion of each subdomain is performed independently. 
% In each subdomain, the dimension of the unknown parameter is reduced and therefore the application of various sampling methods which have limitations in dimensions are enabled.
% Also, this algorithm achieves a reduction in computation cost owing to the parallelization.
% However, this method treats these sub-problems as independent and neglects the implicit relations among local random inputs.
% To exchange information among sub-domains, a globally-informed domain decomposition method is proposed. Take $\bF_C$ be the forward operator over the coarse scale in the global domain and $\bF_F$ be the forward operator over the fine scale in the global domain, and $\bF_F^{(i)}$ denote the forward operator over the fine scale in the $i$-th subdomain.

% Due to uncertain boundary conditions, the local inversion results have larger variance compared to the local problem with accurate boundary conditions.

% In the area of domain decomposition, the information exchange among sub-domains is of crucial importance.
% In the forward computation, the information exchange is achieved via boundary condition iterations. 
% However, in the inverse problems, even though the boundary condition cannot be obtained exactly, we can still give a relatively good initial state using the neighbouring measurements data. 

% First, a stopping criterion based on the boundary condition is proposed. The initial boundary condition is fitted using the data only restricted within the local domain, and due to this reason, the same boundary shared by two subdomains may have different regression result, 

% The globally-informed domain decomposition algorithm we proposed can be easily adjusted to parallelization.

% Communication step among subdomains can greatly slow down the.
% On each subdomain, any classical MCMC method can be used to draw samples from the posterior distribution given the corresponding dataset. 
% Finally, the samples from each subdomain are combined to form samples from the full posterior. 

% The main idea is to borrow the \textit{swap} step to 

\begin{algorithm}[!ht]
    \caption{Domain-Decomposed MCMC method}
    \label{alg:parallel_MCMC}
    \begin{algorithmic}[1]
        \REQUIRE{Dataset $S$, global domain $\calD$, covariance function $C(x,y)$.}
        \STATE{Partition the global domain $\calD$ into $M$ non-overlapping local domains $\{\calD^{(i)}\}_{i=1}^M$.}
        \STATE{Compute the global KL eigenpairs $\{\lambda_r,\psi_r\}_{r=1}^d$  using \eqref{eq:global_eigenpair_1}-\eqref{eq:global_eigenpair_2}.}
        \STATE{Divide the dataset $S$ into $\{S^{(i)}\}_{i=1}^M$, $S^{(i,j)}$ according to domain division}.
        \FOR{every interface $\tau^{(i,j)}$}{
        \STATE{
        Initialize the training data $\Lambda^{(i,j)}:=S^{(i,j)}$, and set $E=1$.}
        \STATE{
        Train the GP model $\widetilde{h}^{(i,j)}:=\mathcal{N}(\mu_{n^{(i,j)}},\sigma_{n^{(i,j)}})$ with $\Lambda^{(i,j)}$ using \eqref{eq:gp_post}}.
        \STATE{Compute the discretized maximum posterior variance $\sigma_{N^{(i,j)}}^{\max}$ using \eqref{eq:max_var}.}
        \WHILE{
        $\sigma_{N^{(i,j)}}^{\max}\ge \delta_{\text{tol}}$ and $\Lambda^{(i,j)}\subset S$}
        \STATE{Update the training data set as $\Lambda^{(i,j)}=S^{(i,j),E\epsilon}$}.
        \STATE{Set $E = E+1$ and go back to line 6.}
        \ENDWHILE
        }
        \STATE{
        Use the posterior mean $\mu_{n^{(i,j)}}$ as the interface condition for $\tau^{(i,j)}$.}
        \ENDFOR
        \STATE{Compute the local KL eigenpairs $\{\lambda_r^{(i)},\psi_r^{(i)}\}_{r=1}^{d^{(i)}}$ for $i=1,\ldots,M$ using  \eqref{eq:local_eigenpair}.} 
        \STATE{Construct the local parameterized forward models $\widetilde{F}_{\text{GP}}^{(i)}$ (see \eqref{eq:local_forward_GP}) for $i=1,\ldots,M$. }
    %\WHILE{Stopping criteria is satisfied}
    \FOR{ subdomain $i=1,\ldots,M$}
    %\STATE{\textcolor{blue}{$\%$ In a parallel manner}}
    \STATE{Run inversion to obtain posterior samples $\{\xi^{(i,k)}\}_{k=1,\ldots,K^{(i)}}$ with partial data $S^{(i)}$ using Algorithm \ref{alg:MHMCMC}.
    (Or other arbitrary sampling methods).}
    \ENDFOR
  \STATE{Assemble the local inversions to get the assembled random field $\widehat{a}$ using \eqref{eq:assembled_kle}.}
  \ENSURE{ The assembled random field $\widehat{a}(x,\widehat{\xi}(\omega))$}.
    \end{algorithmic}
\end{algorithm}

